A Bisimilarity Congruence for the Applied pi-Calculus Sufficiently Coarse to Verify Privacy Properties

This paper is the first thorough investigation into the coarsest notion of bisimilarity for the applied pi-calculus that is a congruence relation: open barbed bisimilarity. An open variant of labelled bisimilarity (quasi-open bisimilarity), better suited to constructing bisimulations, is proven to coincide with open barbed bisimilarity. These bisimilary congruences are shown to be characterised by an intuitionistic modal logic that can be used, for example, to describe an attack on privacy whenever a privacy property is violated. Open barbed bisimilarity provides a compositional approach to verifying cryptographic protocols, since properties proven can be reused in any context, including under input prefix. Furthermore, open barbed bisimilarity is sufficiently coarse for reasoning about security and privacy properties of cryptographic protocols; in constrast to the finer bisimilarity congruence, open bisimilarity, which cannot verify certain privacy properties.

==> late.tex <==
\subsection{Correctness criteria for open bisimilarity for the applied $\pi$-calculus}

Results justifying the soundness of open bisimilarity extend from the $\pi$-calculus to the applied $\pi$-calculus.
Notably open bisimilarity is a congruence.
\begin{theorem}
Open bisimilarity is a congruence.
\end{theorem}

Consequently, open bisimulation is sound with respect to open barbed bisimulation.
\begin{corollary}
Open bisimilarity for the applied $\pi$-calculus is sound with respect to open barbed bisimilarity.
\end{corollary}

Observe that the following are not open bisimilar according to our definition.
\[
 \match{\pair{x}{y} \not= \pair{u}{v}}P 
~~\sim~~
\match{x \not= u}P + \match{y \not= v}P
\qquad
\mbox{where}~
 P \coloneq \mathopen{\tau.}\left(\match{x = u}\cout{x}{x} + \match{y = v}\cout{y}{y}\right)
\]
%The following example reveals a dimension of design decisions in definitions of open bisimulation. 
%By considering each representative disunifying substitution separately, the processes are open bisimilar. However, each disunifier induces unnecessarily strong branching behaviour -- fixing the form of some variables unnecessarily early.
There is a reachable "world" with constraint $\pair{x}{y} \not= \pair{u}{v}$, enabling transition 
$\match{\pair{x}{y} \not= \pair{u}{v}}P \lts{\tau} P$.
In contrast, for the same world where $\pair{x}{y} \not= \pair{u}{v}$, process $\match{x \not= u}P + \match{y \not= v}P$ cannot yet perform any transition without additional assumptions, (Observe $\pair{x}{y} \not= \pair{u}{v} \not\vDash x \not= u$, since $\sub{x}{u}$ respects $\pair{x}{y} \not= \pair{u}{v}$).
Furthermore, in the world where $\pair{x}{y} \not= \pair{u}{v}$, both worlds where $x = u$ and $y = v$ remain reachable, hence both branches of $P$ can be enabled; whereas in the later process either $x \not= u$ or $y \not= v$ and hence a branch of $P$ is permanently disabled.

In contrast, the above processes are open barbed bisimilar, since the context must fix either $x \not= u$ or $y \not= v$; however for the applied $\pi$-calculus these inequalities can be induced in infinitely many ways. 
This example reveals a dimension of design decisions in definitions of open bisimulation. 
Recall ``worlds'' are constraints symbolically representing infinitely many solutions. 
In a sense, there appears to be no canonical choice of ``world'' for open bisimulation, which is determined by a trade of between the granularity and efficiency of equivalence checking.


\paragraph{Strong equivalence.}
Surprisingly, we are unaware of an investigation of late bisimulation in the applied $\pi$-calculus.
Thus in order to properly situate open bisimulation we introduce the following definitions as a reference point.

\begin{definition}[closed labelled transition]
We say a history $h$ grounds processes $P$ whenever all free variables in $P$ appear as outputs in $h$.
A closed labelled transition, $P \clts{\pi} Q$,
is equivalent to $h \colon P \lts{\pi} Q$, according to Fig.~\ref{figure:active} for grounding history $h$. 
% and there are at least as many fresh outputs in $h$ as there are input actions in $P$ and $Q$.
\end{definition}
For the $\pi$-calculus, closed labelled transitions correspond to the classical labelled transition system with mismatch~\cite{Parrow1995}. Thus classically, $\match{x \not= y}\tau \clts{\tau} 0$ always, since late bisimulation assumes free variables are distinct names (constants).
Closed labelled transitions exclusively are employed in the following definition.
%Note here we assume classical labelled transitions system~\cite{Parrow1995}, which can be achieved by performing all tranisitons  by 
\begin{definition}[late bisimulation]
A symmetric relation $\mathrel{\mathcal{R}}$ is a late bisimulation whenever,
if $A \mathrel{\mathcal{R}} B$, then:
\begin{itemize}
\item $A$ and $B$ are statically equivalent.
\item If $A \clts{\tau} A'$ then there exists $B'$ such that $B \clts{\tau} B'$ and $A' \mathrel{\mathcal{R}} B'$.
\item If $A \clts{M(x)} A'$, where $x$ fresh for $A$ and $B$, then there exists $B'$ such that $B \clts{M(x)} B'$ and, for all messages $N$,
$A'\sub{x}{N} \mathrel{\mathcal{R}} B'\sub{x}{N}$.
\item If $A \clts{\co{M}(x)} A'$, where $x$ fresh for $A$ and $B$, then there exists $B'$ such that $B \clts{\co{M}(x)} B'$ and $A' \mathrel{\mathcal{R}} B'$.
\end{itemize}
Late bisimilarity is the greatest late bisimulation.
Strong equivalence is the greatest congruence contained in late bisimilarity.
\end{definition}

Having defined strong equivalence for the applied $\pi$-calculus, we confirm that open bisimilarity is sound with respect to this definition.
\begin{proposition}
Open bisimulation is sound with respect to strong equivalence for the applied $\pi$-calculus.
\end{proposition}


\paragraph{Conservativity with respect to the $\pi$-calculus.}
The definitions of open bisimulation and strong equivalence for applied $\pi$-calculus are further justified, by showing that, when restricted to $\pi$-calculus processes, the established definitions coincides with the new definitions.
\begin{proposition}
Open bisimilarity (respectively strong equivalence) for the applied $\pi$-calculus is a conservative extension of open bisimulation (respectively strong equivalence) for the $\pi$-calculus.
\end{proposition}
The subtlety of the above proposition is that outputs of the form $\co{x}y$ in the $\pi$-calculus become bound outputs in the applied $\pi$-calculus. Static equivalence is then used to distinguish processes.

For example, consider $\pi$-calculus processes $\co{x}y \not\lsim \co{x}x$.
Using applied $\pi$-calculus transitions, a distinguishing strategy is that both processes perform bound output $\co{x}(u)$ reaching the pair of extended processes $\sub{u}{y} \cpar 0 \not\lsim^{x^i\cdot y^i \cdot u^o} \sub{u}{x} \cpar 0$. These extended processes are not statically equivalent, as distinguished by ``recipes'' $u$ and $y$.
Clearly, $\left(u = y\right)\sub{u}{y}$ everywhere.
In contrast, $\left(u \not= y\right)\sub{u}{x}$, unless $x = y$; expressed intuitionistically as $u = y \yields x = y$.
Note that this leads to the following distinguishing formulae.
\[
\co{x}y \vDash \diam{\co{x}(u)}\left(u = y\right)
\qquad
\co{x}x \vDash \boxm{\co{x}(u)}\left(u = y \yields x = y\right)
\]

Similarly, inequation
$\nu z.\left( \co{x}z \cpar \co{x}z \right)
\not\lsim
\nu z.\co{x}z \cpar \nu z.\co{x}z$ 
remains valid for the applied $\pi$-calculus semantics.
The distinguishing strategies according to the applied $\pi$-calculus are explained by the following distinguishing formulae.
\[
\nu z.\left( \co{x}z \cpar \co{x}z \right)
\vDash
\diam{\co{x}(u)}\diam{\co{x}(v)}\left( u = v \right)
\qquad
\nu z.\co{x}z \cpar \nu z.\co{x}z
\vDash
\boxm{\co{x}(u)}\boxm{\co{x}(v)}\left( u \not= v \right)
\]


\paragraph{Generalisation of the spi-calculus.}
Open bisimulation for the applied $\pi$-calculus coincides with open bisimulation for the spi-calculus, as long as the message theory is fixed appropriately.
\begin{proposition}
Open bisimilarity for the applied $\pi$-calculus is a generalisation of open bisimulation for the spi-calculus.
\end{proposition}
The proof of the above propositions is quite involved, since open and late bisimilarity~\cite{briais06entcs,tiu07aplas} for the spi-calculus are typically defined in a different style, using ``hedges''~\cite{borgstrom05mscs}, representing indistinguishable messages exposed to the environment. Following insight from this result, is also possible to define hedged open bisimulation for the applied $\pi$-calculus, which is more involved, but provides a definition closer to an implementation.
 
For comparing the applied $\pi$-calculus to the spi-calculus messages are restricted to the Dolev-Yao model consisting of 
pairs $\pair{M}{N}$, symmetric encryption $\enc{M}{N}$, as assumed by default for the spi-calculus~\cite{abadi99ic}.
We also require the corresponding deconstructors $\fst{M}$, $\snd{M}$ and $\dec{M}{N}$ and,
in order for static equivalence to have the standard distinguishing power of the spi-calculus, 
type checks $\texttt{is\_pair}(\pair{M}{N}) = \ok$,
$\texttt{is\_enc}(\enc{M}{K}) = \ok$
and
$\texttt{can\_dec}(\enc{M}{K},K) = \ok$.
%Restricted to message language $M \coloneqq \pair{M}{N} \mid \enc{M}{N}$
Process in spi-calculus are embedded directly as applied $\pi$-calculus processes by using the following abbreviations.
%Compared to the spi-calculus the let statements that are used to deconstruct messages.
%Such let statements can be encoded using a type check in a guard. For example a let statement deconstructing a pair of messages into it two projections can be encoded as follows.
\[
\begin{array}{rl}
\clet{\pair{x}{y}}{M}{P} \triangleq& \mathopen{\left[\mathrm{is\_pair}(M) = \ok \right]}P\sub{x,y}{\fst{M},\snd{M}}
\\
\ccase{M}{x}{K}{P} \triangleq& \mathopen{\left[\texttt{can\_enc}(M,K) = \ok \right]}P\sub{x}{\dec{M}{K}}
\end{array}
\]
Recall from the discussion surrounding Fig.~\ref{figure:messages}, using an encryption mechanism for which a failed decryption is always detectable can lead to attacks~\cite{Bleichenbacher1998}.
Thus an encryption mechanism satisfying the default theory for the spi-calculus, presented above, is not recommended.
The above discussion is only for strongly situating the applied $\pi$-calculus with respect to the literature on the spi-calculus.


\begin{comment}
If, as in the spi-calculus, we would like a let statement that only succeeds if a decryption is successful, we require an extra message term $\mathrm{can\_decrypt}$
and equation that can detect whether a message decryption is successful. A let statement that only proceeds if a decryption is successful can then be encoded as follows.
\[
 \clet{x}{\adec{M}{K}}{P} \triangleq \mathopen{\left[\mathrm{can\_decrypt}(M,K) = \ok \right]}P\sub{x}{\adec{M}{K}},
\mbox{ where $\mathrm{can\_decrypt}(\aenc{M}{\pk{K}}, K) = \ok$}
\]
Remember though, using an encryption mechanism for which a failed decryption is always detectable can lead to attacks~\cite{Bleichenbacher1998}.
The above encoding is simply intended to show that all constructs from the spi-calculus can be captured in the applied $\pi$-calculus
by adopting a suitable message theory permitting the additional checks the spi-calculus imposes.

The following abbreviation simplify examples.

$\mathopen{\left[\checksign{M,N}{K}\right]}P \triangleq \mathopen{\left[\checksign{M,N}{K} = \ok\right]}P$.

$\cout{x}{M_1, M_2, \hdots M_n} \triangleq \cout{x}{\pair{M_1}{\langle{M_2},{\hdots M_n\rangle \hdots}}}$

$\nu x_1, x_2, \hdots x_n. P \triangleq \nu x_1. \nu x_2. \hdots \nu x_n. P$
\ross{If then else goes here, once mismatch is included.}
\end{comment}



\begin{comment}
\subsection{Soundness with respect to late bisimulation}

\begin{definition}[late bisimulation]
A symmetric relation $\mathrel{\mathcal{R}}$ is a late bisimulation whenever,
if $A \mathrel{\mathcal{R}} B$, then:
\begin{itemize}
\item $A$ and $B$ are statically equivalent.
\item If $A \lts{\tau} A'$ then there exists $B'$ such that $B \lts{\tau} B'$ and $A' \mathrel{\mathcal{R}} B'$.
\item If $A \lts{M(x)} A'$, where $x$ fresh for $A$ and $B$, then there exists $B'$ such that $B \lts{M(x)} B'$ and, for all messages $N$,
$A'\sub{x}{N} \mathrel{\mathcal{R}} B'\sub{x}{N}$.
\item If $A \lts{\co{M}(x)} A'$, where $x$ fresh for $A$ and $B$, then there exists $B'$ such that $B \lts{\co{M}(x)} B'$ and $A' \mathrel{\mathcal{R}} B'$.
\end{itemize}
Late bisimilarity is the greatest late bisimulation.
Late congruence is the greatest congruence contained in late bisimilarity.
\end{definition}


\begin{proposition}
Open bisimulation is sound with respect to late bisimilarity for the applied $\pi$-calculus.
\end{proposition}
\end{comment}


==> modal_proof.tex <==
Since $\sim$ is a greatest fixed point, $\not\sim$ is defined by a least fixed point over a family of symmetric relations satisfying the dual property, where for $\not\sim_n$ a distinguishing stragegy is found withing $n$ transitions.
Note this technique is guaranteed for fragments for which quasi-open bisimilarity is decidable (the question of whether the technique works for undecidable fragments is an open problem).
Thereby, if $P \not\sim Q$, there exists $n \in \omega$ such that $P \not\sim_n Q$, so we can proceed by induction on the depth of a distinguishing strategy.
There are two forms of base case, defining $A \not\sim_0 B$, the first triggered when a labelled transition can only be performed by one process,
the second triggered by static equivalence failing.
The inductive case, defining $A \not\sim_{n+1} B$ is where both processes can act, but all processes reached can be distinguished later in the bisimulation game.


\textbf{Base case involving transition.}
In the first base case the extended progesses, in some reachable world, can be distinguished by one process performing a transition but the other not.
Consider the case where $A$ leads, the case where $B$ leads is symmetric.
For some $\sigma$, $\vec{n}$ and $\rho$, we have $A \leq_{\sigma,\nu \vec{n}.\rho} A'$ and $B \leq_{\sigma,\nu \vec{n}.\rho} B'$
such that $A' \lts{\pi\sigma} C$, but there does not exist $D$ such that $B' \lts{\pi\sigma} Q'$.

Firstly, observe we can identify a set of equalities and inequalities on message, inducing the world reached by substitution $\sigma$ and environment extension $\nu \vec{n}.\rho$ such that $A' \lts{\pi\sigma} C$.
% is applied and the set of names $\vec{m}$ are extended to $\vec{n},\vec{m}$, by using pairs of names.
By unforlding the rules of the labelled transition system for transition $A' \lts{\pi\sigma} C$,
list all pairs of messages in match and mismatch guards as sets of equalities $\mathcal{E}$ and inequalities repectively $\mathcal{D}$.
%There exist finitely many pairs of variables $x_i$ and $y_i$, selected from $\fv{P} \cup \fv{Q} \cup \fv{\alpha}$ such that $x_i\sigma = y_i\sigma$.
%Also, there are  finitely many pairs of variables $w_j$ and $z_j$ such that: either $w_j\sigma \in \vec{n} \setminus \vec{m}$ and $z_j\sigma$ is a distinct variable such that $z_j \in \fv{P} \cup \fv{Q} \cup \fv{\alpha}$, or $\alpha$ is a free input $uz_j$ where $z_j\sigma$ is fresh and $w_j\sigma \in \vec{n}, \vec{m}$ (the second case caters for set of free names being extended by an input transition).

Secondly, we can identify pairs of messages, separating any reachable world in which an $\pi$-transition is enabled for $B$,
for the world $B'$ identified in the distinguishing strategy.
% induced by $\sigma$ and $\vec{n}$, where no $\alpha\sigma$ transition is enabled.
Assume for some $E$, $\varsigma$, $\vec{n}$ and $\varrho$, we have $B \lts{\varsigma,\nu \vec{m}\varrho} \hat{B}$ and $\hat{B} \lts{\pi\varsigma} F$.
Now, as above, unfold the ruels of labelled transtions and gather all equalities and inequalities $\mathcal{E}'$ and $\mathcal{D}'$ enabling $E \lts{\pi\varsigma} F$.
Hence, assuming $B' = \mathopen{\nu k.}\left( \theta \cpar Q \right)$,
either there exists a ``separating'' $\hat{M} = \hat{N} \in \mathcal{E}'$ such that $\hat{M}\sigma\theta =_E \hat{N}\sigma\theta$ does not hold; or there exists ``separating'' $\hat{K} \not= \hat{L} \in \mathcal{D}'$ such that $\vec{k} \vDash K\sigma\theta \not= L\sigma\theta$ does not hold.
To see why, observe that, otherwise, %we have $\mathcal{E}', \mathcal{D}' \leq \mathcal{E}, \mathcal{D}$; hence
any substitution and environment extension satisfying $\mathcal{E}', \mathcal{D}'$ also satisfies $\mathcal{E}, \mathcal{D}$, contradicting the assumption $B'$ has no $\pi\sigma$ transition.
There are only finitely many combinations of $\mathcal{E}'$ and $\mathcal{D}'$ to check, hence we can construct a finite set of separating equlities $\hat{\mathcal{E}}$ and inequalities $\hat{\mathcal{D}}$.

From the above observations, we can construct two distinguishing formulae: $\left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt$ biased to $A$, and $\boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)$ biased to $B$.
There are four cases to check to confirm that these are distinguishing formulae.
\begin{description}
\item[{Case} $A \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt\,$:]
Assume $\varsigma$, $\vec{a}$, $\vec{b}$, $\varrho$, $\theta$ and $P$ such that $\theta$ $A \leq_{\varsigma,\nu \vec{a}.\varrho} \mathopen{\nu \vec{b}.}\left( \theta \cpar P\right)$, 
and, for all $M = N \in \mathcal{E}$, we have $M\varsigma\theta =_E N\varsigma\theta$,
and also, for all $K \not= L \in \mathcal{D}$, we have $\vec{b} \vDash K\varsigma\theta \not= L\varsigma\theta$.
%Hence, for all extended processes $F$, $\vec{b}.\left( \theta \cpar F\right) \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right)\mathclose{\varsigma}$.
Since every equation and inequation enabling $A' \lts{\pi\sigma} C$ must also be enabled for $\mathopen{\nu\vec{b}.}\left( \theta \cpar P\right)$
we have, for some extended process $F$, $\mathopen{\nu\vec{b}.}\left( \theta \cpar P\right) \lts{\pi\varsigma} F$, and trivially $F \vDash \ttt$.
Thereby $\mathopen{\nu\vec{b}.}\left( \theta \cpar F\right) \vDash \diam{\pi\varsigma}\ttt$ holds, by definition of the diamond modality.
Hence, by definition of implication, we have $A \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt$, as required.

\item[{Case} $B \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt\,$:]
Assume for contradiction $B \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt$.
Since $B \leq_{\sigma,\nu \vec{n}.\rho} B'$, the above holds
only if $B' \vDash \diam{\pi\sigma}\ttt$ holds,
which holds only if there exists extended process $D$ 
such that $B' \lts{\pi\sigma} D$, contradicting the assumption that no such $D$ exists.
Thereby, we have $B \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt$.

\item[{Case} $B \vDash \boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)\,$:]
Assuming $B \leq_{\varsigma,\nu \vec{a}.\varrho} \nu \vec{b}.\left( \theta \cpar Q\right)$
and $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \lts{\pi\varsigma} \hat{B}$, for some $\hat{B}$.
In this scenario, as argued above, we have either: for some $\hat{M} = \hat{N} \in \hat{\mathcal{E}}$ we have $\hat{M}\varsigma\theta =_E \hat{N}\varsigma\theta$;
or, for some $\hat{K} \not= \hat{L} \in \hat{\mathcal{D}}$, we have $\vec{b} \vDash \hat{K}\varsigma\theta \not= \hat{L}\varsigma\theta$.
Thus, either: for some $\hat{M} = \hat{N} \in\hat{\mathcal{E}}$ we have $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \vDash M\varsigma = N\varsigma$ and so $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \vDash \bigvee \hat{\mathcal{E}}\varsigma$;
or, for some $\hat{K} \not= \hat{L} \in \hat{\mathcal{D}}$ we have $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \vDash M\varsigma \not= N\varsigma$ and so $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \vDash \bigvee \hat{\mathcal{D}}\varsigma$.
Thereby, in either case, we have $\mathopen{\nu\vec{b}.}\left( \theta \cpar Q\right) \vDash \left(\bigvee \hat{\mathcal{E}} \vee \bigvee \hat{\mathcal{D}}\right)\mathclose{\varsigma}$.
Thereby, by definition of $\boxm{\pi}$ we have established
$B \vDash \boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)$.

\item[{Case} $A \not\vDash \boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)\,$:]
Assume for contradiction $A \vDash \boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)$ holds.
Since $A \leq_{\sigma,\nu \vec{n}.\rho} A'$  and $A' \lts{\pi\sigma} C$
it must have been the case that
$C \vDash \left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)\mathclose{\sigma}$.
This holds only if either: for some $\hat{M} = \hat{N} \in \mathcal{E}$ we have $C \vDash \hat{M}\sigma = \hat{N}\sigma$;
or, for some $\hat{K} \not= \hat{L} \in \mathcal{D}$ we have $C \vDash \hat{K}\sigma \not= \hat{L}\sigma$.
Now assume $C = \mathopen{\nu \vec{d}.}\left( \vartheta \cpar R \right)$, fo some $\vec{d}$, $\vartheta$ and $R$.
Consequently either: for some $\hat{M} = \hat{N} \in \hat{\mathcal{E}}$ we have $\hat{M}\sigma\vartheta =_E \hat{N}\sigma\vartheta$;
or for some $\hat{K} \not= \hat{L} \in \hat{\mathcal{D}}$ we have $\vec{d} \vDash \hat{K}\sigma\vartheta \not= \hat{L}\sigma\vartheta$.
The constradicts the assumptions behind the construction of $\hat{\mathcal{E}}$ and $\hat{\mathcal{D}}$.
Thereby $A \not\vDash \boxm{\pi}\left(\bigvee{\hat{\mathcal{E}}} \vee \bigvee\hat{\mathcal{D}}\right)$.
\end{description}


\textbf{Base case for static equivalence.}
In the second base case, in some reachable world, $A$ and $B$ are not statically equivalent.
That is there exist $\sigma$, $\vec{a}$, $\rho$ such that $A \leq_{\sigma,\nu\vec{a}.\varsigma} \mathopen{\nu \vec{x}.}\left(\theta \cpar P\right)$ and $B \leq_{\sigma,\nu\vec{a}.\rho} \mathopen{\nu \vec{y}.}\left(\rho \cpar Q\right)$ and $\mathopen{\nu \vec{x}.}\left(\theta \cpar P\right)$ is not statically equivalent to $\mathopen{\nu \vec{y}.}\left(\rho \cpar Q\right)$,
and without loss of generality $\sigma$ is fresh for $\vec{x}\cup\vec{y}$ (applying $\alpha$-conversion).
By definition of static equivalence, there exist messages $M$ and $N$ such that $M\sigma\theta =_E N\sigma\theta$ holds but $M\sigma\rho =_E N\sigma\rho$ does not hold (or conversely with $\theta$ and $\rho$ interchanged).
We can construct a set of equalities $\mathcal{E}$ as $\left\{z_1 = K_1, \hdots, z_n = K_n\right\}$ 
where $\sigma = \sub{z_1, \hdots, z_n}{K_1,\hdots K_n}$.
Thereby we have $A \vDash \bigwedge\mathcal{E} \yields M = N$,
but $B \not\vDash \bigwedge\mathcal{E} \yields M = N$,
since $\mathopen{\nu \vec{y}.}\left(\rho \cpar Q\right) \vDash \mathcal{E}\sigma$, but $\mathopen{\nu \vec{y}.}\left(\rho \cpar Q\right) \not\vDash M\sigma = N\sigma$.

Also we can construct sets of equalities $\hat{\mathcal{E}}$ such that,
for all $\varrho$ fresh for $\dom{\theta}$, and w.l.o.g.\ fresh for $\vec{x}\cup\vec{y}$, such that $M\sigma\varrho\rho =_E N\sigma\varrho\rho$,
we have there exists $\hat{K} = \hat{L} \in \hat{\mathcal{E}}$ such that $\hat{K}\sigma\varrho =_E \hat{L}\sigma\varrho$, but $\hat{K}\sigma$ is distinct from $\hat{L}\sigma$.
%To see why, observe that it is impossible that for all pairs of messages $\hat{M}$ and $\hat{N}$ such that $\left(\fv{\hat{M}}\cup\fv{\hat{N}}\right)\cap\left(\dom{\theta} \cup \vec{x}\cup\vec{y}\right) = \emptyset$ and $\hat{M}\sigma\varrho =_E \hat{N}\sigma\varrho$ we have $\mathcal{M}\sigma =_E \mathcal{N}\sigma$.
%, but $K\sigma\theta\varrho$ is distinct from $\hat{L}\sigma\theta\varrho$.
Assuming the equational theory is finitary, a finite $\hat{\mathcal{E}}$ exists.
Hence $B \vDash \bigwedge\mathcal{E} \yields M = N \yields \bigvee\hat{\mathcal{E}}$. 
% \vee \bigvee\hat{\mathcal{D}}$,
However, $A \not\vDash \bigwedge\mathcal{E} \yields M = N \yields \bigvee\hat{\mathcal{E}}$,
since $\mathopen{\nu \vec{y}.}\left(\theta \cpar P\right) \vDash \mathcal{E}\sigma$ and $\mathopen{\nu \vec{y}.}\left(\theta \cpar P\right) \vDash M\sigma = N\sigma$, but $\mathopen{\nu \vec{y}.}\left(\theta \cpar P\right) \not\vDash \hat{K}\sigma = \hat{L}\sigma$, for all $\hat{K} \not= \hat{L} \in \hat{\mathcal{M}}$, thereby $\mathopen{\nu \vec{y}.}\left(\theta \cpar P\right) \not\vDash \bigvee\hat{M}\sigma$, as required.
% \vee \bigvee\hat{\mathcal{D}}$.
%for all $K = L \in \mathcal{E}$ we have $K\sigma\rho =_E N\sigma\rho$,
%and for all $K' \not= L' \in \mathcal{D}$ we have $\vec{x} \vDash K'\sigma\rho \not= L'\sigma\rho$.


\textbf{Inductive case.}
The inductive case is similar in construction to the base case when one process leads with a transition, but requires some additional assumptions ensuring we select a distinguishing strategy that is in some sense minimal.
Whenever $A \not\sim_{n+1} B$, up to symmetry of $\not\sim_{n+1}$, we have the following.
\begin{itemize}
\item For some $\sigma$, $\vec{a}$, $\rho$, $C$ such that $A \leq_{\sigma,\nu \vec{a}.\rho} A'$
and $B \leq_{\sigma,\nu \vec{a}.\rho} B'$ and also $A' \lts{\pi\sigma} C$, 
we have, for all $D_i$ such that $B' \lts{\alpha\sigma} D_i$, we have $C \not\sim_n D_i$.
\end{itemize}
%such that $\vec{n}, \vec{m} \colon Q\sigma \lts{\co{a\sigma}(z)} Q_i$.
%For each $i$, $P' \not\sim^{\vec{n}, \vec{m}, z}_n Q_i$, 
Observe, by image-finiteness upto $\alpha$-conversion, there exist finitely many such $D_i$.
Furthermore, by the induction hypothesis, there exist $\phi^L_i$ and $\phi^R_i$ 
such that $C \vDash \phi^L_i\sigma$ and $D_i \not\vDash \phi^L_i \sigma$
and $C \not\vDash \phi^R_i \sigma$ and $D_i \vDash \phi^R_i \sigma$.



%By Lemma~\ref{lemma:sub},
By a similar argument to the base case, 
there exist finite sets of pairs of messages $\mathcal{E}$ and $\mathcal{D}$, read from the rules of the labelled transition,
such that enabling transition $A' \lts{\pi} C$ and $C \vDash \phi^L_i$, 
and, furthermore, 
under all subtitutions and environment extension for which $\mathcal{E}$ and $\mathcal{D}$ hold, the transition is enabled and satisfaction holds
(i.e.\ if $A \leq_{\varsigma,\nu\vec{e}.\varrho} F$ and $F \vDash \left(\bigwedge\mathcal{E}\wedge \bigwedge\mathcal{D}\right)\mathclose{\varsigma}$ we have $F \lts{\pi\varsigma} G$ and $G \vDash \phi^L_i\varsigma$).

Also there exist finite sets of pairs of message $\hat{\mathcal{E}}$ and $\hat{\mathcal{D}}$ 
such that for all $\varsigma$, $\rho$, $\theta$, $\vec{b}$ and $\hat{A}$
such that $A \leq_{\varsigma,\nu \vec{b}.\rho} \mathopen{\nu \vec{c}.}\left( \vartheta \cpar R \right)$
and $C = \mathopen{\nu \vec{d}.}\left( \theta \cpar Q \right)$ we have, the following:
\begin{itemize}
\item Either, for some $\phi^R_i$ we have $\mathopen{\nu \vec{c}.}\left( \vartheta \cpar R \right) \vDash \rho^R_i$;

\item or, for some $\hat{M} = \hat{N} \in \hat{\mathcal{E}}$ we have $\hat{M}\varsigma\vartheta =_E \hat{N}\varsigma\vartheta$ holds but $\hat{M}\sigma\theta =_E \hat{N}\sigma\theta$ does not hold;

\item or, for some $\hat{K} \not= \hat{L} \in \hat{\mathcal{D}}$ we have $\vec{c} \vDash \hat{K}\varsigma\vartheta \not= \hat{N}\varsigma\vartheta$ holds but $\vec{d} \vDash \hat{K}\sigma\theta \not= \hat{L}\sigma\theta$ does not hold.
\end{itemize}

Using the above sets of pairs of message, we can construct a pair of distinguishing formulae: $\left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\bigwedge_i \phi^L_i$ is 
biased to $A$ and
$\left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$ biased to $B$.
There are four cases to consider to verify these are indeed distinguishing formulae.
\begin{description}%[leftmargin=2.5mm]

\item[{Case} $A \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\bigwedge_i \phi^L_i$\,:]
Assume $\varsigma$, $\vec{a}$, $\vec{b}$, $\varrho$, $\theta$ and $P$ are such that $A \leq_{\varsigma,\nu \vec{a}.\varrho} \mathopen{\nu\vec{b}.}\left( \theta \cpar P\right)$
and, for all $M = N \in \mathcal{E}$, we have $M\varsigma\theta =_E N\varsigma\theta$,
and also, for all $K \not= L \in \mathcal{D}$, we have $\vec{b} \vDash K\varsigma\theta \not= L\varsigma\theta$.
Since every equation and inequation enabling $A' \lts{\pi\sigma} C$ must also be enabled for $\mathopen{\nu\vec{b}.}\left( \theta \cpar P\right)$
we have, for some extended process $F$, $\mathopen{\nu \vec{b}.}\left( \theta \cpar P\right) \lts{\pi\varsigma} \mathopen{\nu\vec{b}.}\left( \theta \cpar F\right)$
(without loss of generality, we can assume if $\pi = \co{M}(u)$, we have $\varsigma$ is fresh for $u$).
Furthermore, since $\mathopen{\nu\vec{b}.}\left( \theta \cpar P\right) \vDash \bigwedge\mathcal{E}\varsigma$  since $\mathopen{\nu\vec{b}.}\left( \theta \cpar F\right) \vDash \phi^L_i\varsigma$, by the assumptions on $\mathcal{E}$ and $\mathcal{D}$.
%$\mathopen{\nu\vec{b}.}\left( \theta \cpar F\right) \vDash \phi^L_i\varsigma$.
Thereby $\mathopen{\nu\vec{b}.}\left( \theta \cpar F\right) \vDash \diam{\pi\varsigma}\ttt$ holds, by definition of the diamond modality.
Hence, by definition of implication, we have $A \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\ttt$, as required.


\item[{Case} $B \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\bigwedge_i \phi^L_i$\,:]
Suppose, for contradition, 
$B \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\bigwedge_i \phi^L_i$ holds.
Since $B \leq_{\sigma,\nu\vec{a}.\rho} B'$ and $B' \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right)\mathclose{\sigma}$ holds,
the above assumption holds 
only if $B' \vDash \left(\diam{\pi}\bigwedge_i \phi^L_i\right)\mathclose{\sigma}$.
In turn, this holds 
only if there exists $D$ such that
$B' \lts{\co{\pi\sigma}} D$ and 
we have $D \vDash \bigwedge_i \phi^L_i \sigma$,
which holds only if, for all $i$, we have
$D \vDash \phi^L_i \sigma$.
Notice that $D = D_k$ for some $k$,
so it must be the case that $D_k \vDash \phi^L_k \sigma$;
but it was assumed that $D_k \not\vDash \phi^L_k \sigma$, yielding a contradiction.
Therefore $B \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \diam{\pi}\bigwedge_i \phi^L_i$.

\item[{Case} $B \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$\,:]
Fix $\varsigma$, $\vec{a}$, $\varrho$, $\theta$, $Q$ and $\vec{m}$
such that $B \leq_{\varsigma,\nu\vec{a}.\varrho} \mathopen{\nu\vec{m}.}\left( \theta \cpar Q\right)$
such that $\mathopen{\nu\vec{m}.}\left( \theta \cpar Q\right) \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right)\varsigma$ 
%\ross{Check name on $\pi$, without loss of generality assume $z$ is fresh such that $z \not\in \dom{\theta}$ and $z \not\in \vec{n}', \vec{m}$.}
%There are two sub-cases to consider.
By construction of $\hat{\mathcal{E}}$ and $\hat{\mathcal{D}}$ we have:
\begin{itemize}
\item either, for some $\phi^R_i$ we have $\mathopen{\nu \vec{m}.}\left( \vartheta \cpar R \right) \vDash \rho^R_i$;
\item or, for some $\hat{M} = \hat{N} \in \hat{\mathcal{E}}$ we have $\hat{M}\varsigma\vartheta =_E \hat{N}\varsigma\vartheta$ holds, hence $\mathopen{\nu \vec{m}.}\left( \vartheta \cpar R \right) \vDash \hat{M}\varsigma = \hat{N}\varsigma$;
\item or, for some $\hat{K} \not= \hat{L} \in \hat{\mathcal{D}}$ we have $\vec{m} \vDash \hat{K}\varsigma\vartheta \not= \hat{N}\varsigma\vartheta$ holds, hence $\mathopen{\nu \vec{m}.}\left( \vartheta \cpar R \right) \vDash \hat{K}\varsigma \not= \hat{L}\varsigma$.
\end{itemize}
Hence we have $\mathopen{\nu \vec{m}.}\left( \vartheta \cpar R \right) \vDash \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}}$ holds, by definition of disjunction.
Thus, by definition of box and implication,
%$\boxm{\co{a}(z)}$,
$B \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$.


\item[Case $A \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$\,:]
Now assume for contradiction that $A \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$ holds.
Now observe $A \leq_{\sigma,\nu \vec{a}\rho} A'$
and $A' \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right)\sigma$
%Fix $\varsigma$, $\vec{a}$, $\varrho$, $\theta$, $P$, $\vec{m}$ and $F$
%such that $B \leq_{\varsigma,\nu\vec{a}.\varrho} \nu \vec{m}.\left( \theta \cpar P\right)$
%such that $\nu \vec{m}.\left( \theta \cpar P\right) \vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right)\varsigma$
%and $\nu \vec{m}.\left( \theta \cpar P\right) \lts{\pi\varsigma} \nu \vec{m}.\left( \theta \cpar F\right)$.
%Since $\sigma$ respects $\vec{m}$, and we have transition $\vec{n}, \vec{m} \colon P\sigma \lts{\co{a\sigma}(z)} P'$,
Hence the above holds only if $A' \vDash \left(\mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)\right)\mathclose{\sigma}$.
So since $A' \lts{\pi\sigma} C$, where $C = \mathopen{\nu \vec{d}.}\left( \theta \cpar Q \right)$,
the above holds only if
$C \vDash \left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)\mathclose{\sigma}$.
However, we have, $C \not\vDash \phi^R_i$, for all $i$.
Also,
 for all $\hat{M} = \hat{N} \in \hat{\mathcal{E}}$ we have $\hat{M}\sigma\theta =_E \hat{N}\sigma\theta$ does not hold; hence $C \not\vDash M\sigma = N\sigma$.
Similarly, for all $\hat{K} = \hat{L} \in \hat{\mathcal{D}}$ we have $\vec{d} \not\vDash \hat{K}\sigma\theta =_E \hat{N}\sigma\theta$ does not hold; hence $C \not\vDash M\sigma\theta = N\sigma\theta$.
Thus we arrive at a contradiction; hence we have 
$A \not\vDash \left(\bigwedge\mathcal{E} \wedge \bigwedge\mathcal{D}\right) \yields \mathopen{\boxm{\pi}}\left( \bigvee_i \phi^R_i \vee \bigvee\hat{\mathcal{E}} \vee \bigvee\hat{\mathcal{D}} \right)$, as required.
\end{description}

By induction, we have established that, for any $n$, if $A \not\sim_n B$ then 
there exists $\phi_L$ such that $A \vDash \phi_L$ and $B \not\vDash \phi_L$, and also 
there exists $\phi_R$ such that $B \vDash \phi_R$ and $A \not\vDash \phi_R$.
Coincidence with open barbed bisimilarity follows by Corollary~3.9, so if $P \not\bsim Q$, then $P \not\sim Q$;
and, since $\not\sim$ is the least relation containing all $\not\sim_n$,
for some $m$, we have $P \not\sim_m Q$. Thereby 
there exists $\phi_L$ such that $P \vDash \phi_L$ and $Q \not\vDash \phi_L$, and also 
there exists $\phi_R$ such that $Q \vDash \phi_R$ and $P \not\vDash \phi_R$, as required.



==> pilts.tex <==
\section{
Respectful substitutions and 
a late transition system for the $\pi$-calculus with mismatch
}

This section presents a dialect of the $\pi$-calculus with mismatch.
The labelled transition semantics are extended in a minimal fashion in order to evaluate mismatch for open terms, where names are variables rather than distinct constants.
In order to do evaluate mismatch, we require a notion of \textit{respectful substitution} critical throughout this work.

The syntax presented below is standard.
\[
\begin{array}{rlr}
M, N \Coloneqq& x,z & \mbox{messages are variables} \\
\\
\pi \Coloneqq & \tau      & \mbox{progress} \\
         \mid & \co{M}{N} & \mbox{free output} \\
         \mid & \co{M}(z) & \mbox{output} \\
         \mid & M(z)      & \mbox{input} \\
\end{array}
\begin{array}{rlr}
P, Q \Coloneqq& 0 & \mbox{deadlock} \\
          \mid& \pi.P & \mbox{prefix} \\
%          \mid& \cin{x}{y}.P & \mbox{receive} \\
          \mid& \mathopen{\left[M \mathrel{=} N\right]}P & \mbox{match} \\
          \mid& \mathopen{\left[M \not= N\right]}P & \mbox{mismatch} \\
          \mid& \mathopen\nu x. P & \mbox{new} \\
          \mid& P \cpar Q & \mbox{parallel} \\
          \mid& P + Q & \mbox{choice} 
%          \mid& \bang P & \mbox{replication} 
\end{array}
\]
A process can be prefixed by an action, where actions can be silent progress $\tau$, or an input or output action on a channel. An input action $x(z)$ receives on channel $x$ some value symbolically represented by $z$. Output actions can either be free $\co{x}y$ or bound $\co{x}(z)$, in the former $y$ is some public information, but in the later $z$ is a fresh private name.
The private names are bound by the $\nu$ quantifier restricting their scope and freshness.
Processes can be composed in parallel $\cpar$ and choice $+$.
Further to the match guard that passes if two variables are the same, we include a mismatch that passes only if we are certain two varaibles can never be equal.
Note $\match{x=y}P + \match{x\not=y}Q$ encodes $\texttt{if}\,x = y\,\texttt{then}\,P\,\texttt{else}\,Q$.

For the standard $\pi$-calculus in all the following definitions, the messages ranged over by $M$ and $N$ can only be variables $x, y$. 
The definitions in this section use messages, so that they can be reused later in this paper for calculi that permit more general messages.

For open bisimulation, there is no need to syntactically distinguish between names and variables. The different semantic treatments of variables (input variables, bound variables, extruded variables) are distinguished by the environment rather than the syntax.
In particular, open bisimulation disposes of a \textit{distinct name assumption} assumed for classical notions of bisimulation such as late bisimulation.

The environment required to distinguish messages is given by a history and a set of inequalities.
A history represent the order in which private names are extruded ($x^o$) and messages are input ($z^i$).
\begin{definition}[history]
A history is defined by the following grammar, where $x$ is a variable and $M$ is a message:
$h \coloneqq \epsilon \mid h \cdot x^o \mid h \cdot M^i$.
\end{definition}

For the $\pi$-calculus, a history can be represented as a set of inequalities between names, called a \textit{distinction}.
For example, history $w^i \cdot x^o \cdot y^i \cdot z^o$ induces inequalities $x \not= y$, $z \not= w$, $z \not= x$ and $z \not= y$. We adopt histories since histories generalise directly to the applied $\pi$-calculus, where a finite history can represent an infinite number of message inequalities. Furthermore, histories are directly related to the use of universal and nominal quantifiers used in logical embeddings of open bisimulation~\cite{tiu10tocl}.

\begin{comment}
Although histories are employed to handle private names, distinctions are still required for mismatch. Distinctions are used to induce ``worlds'' in which messages are distinguished.

\begin{definition}[distinction and environment]
A distinction $\mathcal{E}$ is a set of pairs of distinct messages, used to symbolically represent inequalities $\left\{ M_1 \not= N_1, \hdots M_k \not= N_k \right\}$.
A distinction-history pair is called an \textit{environment}.
\end{definition}
\end{comment}

The notion of a respectful substitution is required to define reachable ``worlds'' in open bisimulation and the logic $\mathcal{OM}$.
\begin{definition}[respects]
Substitution $\sigma$ respects environment $ h$ iff:
%\begin{itemize}
%\item 
for all $h'$ and $h''$ such that
$h = h'\cdot x^o \cdot h''$,
$\sigma x = x$
and
$y \in \fv{h'}$
implies $x \not \in y\sigma$.
%\item There is no inequality $M \not= N \in \mathcal{E}$ such that $M\sigma = N\sigma$.
%\end{itemize}
\end{definition}
For example substitution $\sub{x}{z}$ does not respect $x^i\cdot z^o$, since $x$ was input before private name $z$ was revealed. 
In contrast, $\sub{x}{z}$ respects history $z^o\cdot x^i$, since private name $z$ was output before $x$ was input. 

Respectful substitutions are used to define a notion of entailment, where the absence of a respectful substitution is used as evidence that messages are always distinct.
\begin{definition}[entailment]
Given history %environment $\mathcal{E}$,
$h$ and messages $M$ and $N$,
entailment $h \vdash M \not= N$ holds whenever,
there is no substitution $\sigma$ respecting $h$ such that $M\sigma = N\sigma$. % in the equational theory.
\end{definition}
For example, since $\sub{x}{z}$ does not respect $x^i\cdot z^o$,
entailment $x^i\cdot z^o \vDash x \not= z$ holds.
%Similarly, if $x\sigma = z\sigma$ then $\sigma$ does not respect $z \not= x$, and hence entailment $z \not= x \vDash x \not= z$ holds.
%Entailment can be generalised to more general constraints, as in the $\psi$-calculus. However, here we present what is necessary for mismatch guards.

\begin{figure}[h!]
%\begin{minipage}
\[
\begin{gathered}
%F \Coloneqq& \mathopen{\left(x\right)}.\mathclose{P} & \mbox{abstraction}
%\begin{array}{rlr}
\begin{array}{c}
\begin{prooftree}
\bn{\pi} \cap \fv{h,\pi} = \emptyset
\justifies
 h \colon \mathopen{\pi.}P \lts{\pi} P
\using
\mbox{\textsc{Act}}
\end{prooftree}
\qquad
\begin{prooftree}
 h \colon P \lts{\co{M}x} Q
\quad
x \not\in \fv{h,M}
\justifies
 h \colon \nu x.P \lts{\co{M}(x)} Q
\using
\mbox{\textsc{Open}}
\end{prooftree}
%\qquad\qquad
%\begin{prooftree}
%\justifies
% h \colon \cout{x}{y}.P \lts{\co{x}y} P
%\using
%\mbox{output}
%\end{prooftree}
\\[15pt]
\begin{prooftree}
 h \colon P \lts{\pi} Q
\justifies
 h \colon {\mathopen{\left[M=M\right]}{P}\lts{\pi}{Q}}
\using
\mbox{\textsc{Mat}}
\end{prooftree}
\qquad
\begin{prooftree}
 h \colon P \lts{\pi} Q
\quad
 h \vDash M \not= N
\justifies
 h \colon {\mathopen{\left[M \not= N\right]}{P}\lts{\pi}{Q}}
\using
\mbox{\textsc{Mismatch}}
\end{prooftree}
\\[15pt]
\begin{prooftree}
 h \colon P \lts{\pi} R
\justifies
 h \colon P + Q \lts{\pi} R
\using
\mbox{\textsc{Sum-l}}
\end{prooftree}
\qquad
\begin{prooftree}
h\cdot x^o \colon P \lts{\pi} Q
\quad
x \not\in \mathrm{n}(\pi,h)
\justifies
 h \colon {{\nu x.P}\lts{\pi}{\nu x.Q}}
\using
\mbox{\textsc{Res}}
\end{prooftree}
\\[15pt]
\begin{prooftree}
 h \colon {P \lts{\pi} Q}
\quad
\fv{R} \cap \bn{\pi} = \emptyset
\justifies
 h \colon {{P \cpar R} \lts{\pi} {Q \cpar R}}
\using
\mbox{\textsc{Par-l}}
\end{prooftree}
\\[15pt]
\begin{prooftree}
 h \colon P \lts{\co{M}(x)} P'
\quad
 h \colon Q \lts{M(x)} Q'
\justifies
 h \colon {P \cpar Q}\lts{\tau}{\mathopen{\nu x.}\left(P' \cpar Q'\right)} 
\using
\mbox{\textsc{Close-l}}
\end{prooftree}
\\[15pt]
\begin{prooftree}
 h \colon P \lts{\co{M}N} P'
\quad
 h \colon Q \lts{M(x)} Q'
%\quad x \not\in\fv{A}
\justifies
 h \colon {P \cpar Q}\lts{\tau} P' \cpar Q'\sub{x}{N}
\using
\mbox{\textsc{Comm-l}}
\end{prooftree}
\end{array}
\end{gathered}
\]
\caption{A late transition semantics for finite $\pi$-calculus processes with mismatch, plus symmetric rules for parallel composition.
The free variables $\fn{}$, bound variables $\bn{}$ and variables $\n{}$ are defined such that: $\fn{M(y)} = \n{\co{M}(y)} = \fn{M}$; $\fn{\co{M}N} = \fn{M}\cup \fv{N}$;
$\bn{M(x)} = \bn{\co{M}(x)} = \left\{ x \right\}$; $\fn{\tau} = \bn{\tau} = \bn{\co{M}{N}} = \emptyset$; $\n{\pi} = \fv{\pi} \cup \bn{\pi}$;
and $\alpha$-conversion is such that $M(x).P$, $\co{M}(x).P$ and $\nu x.P$ bind $x$ in $P$.}\label{figure:pi}
\end{figure}

The late transition semantics in Fig.~\ref{figure:pi} differ only slightly from the standard late transition semantics for the $\pi$-calculus.
Each rule is tagged with an environment consisting of distinctions and a history.
However, the environment information only play a significant role in the rules \textsc{Mismatch} and \textsc{Res}.
The \textsc{Act} and \textsc{Open} rules have extra conditions that simply ensure that bound names on labels are fresh, by ensuring they not get confused with names in the history.

\paragraph{The \textsc{Mismatch} rule.}
Without environment information no process guarded with mismatch can make progress.
A history, such as $x^i\cdot z^o$ can be used to resolve a mismatch such as the following.
\[
\begin{prooftree}
\begin{prooftree}
\justifies
x^i\cdot z^o \colon \tau \lts{\tau} 0
\end{prooftree}
\qquad
x^i\cdot z^o \vDash x \not= z
\justifies
x^i\cdot z^o \colon \match{x \not= z}\tau \lts{\tau} 0
\end{prooftree}
\]
%A similar effect can be achieved by the distinction $x \not= z$, thereby enabling $x \not= z \colon \match{x \not= z}\tau \lts{\tau} 0$.

\paragraph{The \textsc{Res} rule.}
Notice that the \textsc{Res} rule extends the history with a fresh name.
This is essential for resolving a mismatch in which a variable is bound by a $\nu$ quantifier, as in the following example rule instance.
\[
\begin{prooftree}
x^i\cdot z^o \colon \match{x \not= z}\tau \lts{\tau} 0
\justifies
x^i \colon \nu z. \match{x \not= z}\tau \lts{\tau} 0
\end{prooftree}
\]
%Notice that the history covers all free variables in the process on the left of the labelled transition.

\paragraph{Abbreviation for open transitions.}
The free variables in the process on the left of a labelled transition should be covered by the variables appearing in the history. 
%For example, $y^i \colon \nu x.\match{x \not= y}\tau \lts{\tau} 0$, since the operation semantics accumulate the history $y^i \cdot x^o$, for which no substitution equating $x$ and $y$ is respectful.
The following abbreviation implicitly covers variables by inputs:
%\begin{definition}[abbreviation]
$P \lts{\pi} Q$
abbreviates
$\emptyset, x_1^i\cdot\hdots\cdot x_n^i \colon P \lts{\pi} Q$,
where
$\left\{ x_1, \hdots, x_n \right\} \subseteq \fv{P}$.
%\end{definition}
For example $\nu x.\match{x \not= y}\tau \lts{\tau} 0$ is enabled.



==> pimodal.tex <==
\section{Intuitionistic modal logic characterising open bisimilarity for $\pi$-calculus with mismatch}

The intuitionistic modal logic $\mathcal{OM}$ is proven to characterise a finite fragment of the $\pi$-calculus~\cite{Ahn2017}. Here we present a version of $\mathcal{OM}$ that makes fuller use of the power of intuitionistic logic in order to characterise the finite $\pi$-calculus with mismatch.

A syntax for $\mathcal{OM}$ is presented below.
\begin{gather*}
\begin{array}{l}
\left.
\begin{array}{rlr}
\phi \Coloneqq& \ttt & \mbox{top} \\
          \mid& \fff & \mbox{bottom} \\
          \mid& M = N & \mbox{equality} \\
%          \mid& \diam{M = N}\phi & \mbox{diamond match} \\
%          \mid& \diam{M \not= N}\phi & \mbox{diamond mismatch}\\
%          \mid& \boxm{M = N}\phi & \mbox{box match}\\
%          \mid& \boxm{M \not= N}\phi & \mbox{box mismatch}\\
          \mid& \phi \wedge \phi & \mbox{conjunction} \\
          \mid& \phi \vee \phi & \mbox{disjunction} \\
          \mid& \phi \yields \phi & \mbox{implication} \\
\end{array}
\right\}
\mbox{intuitionistic logic}
\\
\left.
\begin{array}{rlr}
\hspace{17pt}
          \mid& \diam{\pi}\phi & \hspace{21pt} \mbox{diamond} \\
          \mid& \boxm{\pi}\phi & \mbox{box}
\end{array}
\right\}
\mbox{modalities}
\end{array}
\begin{array}{l}
\mbox{common abbreviations:}
\\[4pt]
\neg \phi \triangleq \phi \yields \fff
\\
M \not= N \triangleq \neg (M = N)
\\
\boxm{M = N}\phi \triangleq M = N \yields \phi
\\
\diam{M = N}\phi \triangleq M = N \wedge \phi
\\
\boxm{M \not= N}\phi \triangleq M \not= N \yields \phi
\\
\diam{M \not= N}\phi \triangleq M \not= N \wedge \phi
\end{array}
\end{gather*}
In the syntax above, observe connectives cover the standard conjunction, disjunction, implication, top and bottom of intuitionistic logic with equalities. 
The two modalities box and diamond range over all observable actions.
Observable actions $\pi$, as defined previously for the $\pi$-calculus, range over $\tau$, inputs, bound outputs and free outputs. For the $\pi$-calculus messages $M$ range over variables, but will be instantiated in a more general fashion later in this work.
Negative connectives and common constructs for Hennessy-Milner logic are defined as abbreviations.

The semantics of $\mathcal{OM}$ is presented in Fig.~\ref{figure:OM}.
Satisfaction is defined as follows.
\begin{definition}
Process $P$ satisfies formula $\phi$, written $P \vDash \phi$, whenever, according to Fig.~\ref{figure:OM},
$P \vDash^{x_1^i \cdot x_2^i \cdots x_m^i} \phi$
for
$\fv{P} \cup \fv{\phi} \subseteq \left\{ x_1, x_2, \hdots, x_m \right\}$.
\end{definition}

As standard for intuitionistic logic, there is no rule for bottom or equalities between distinct messages (there is no proof of the absurdity). 
Implication is interpreted intuitionistically by checking that the implication holds in worlds reachable by respectful substitutions. Consequently, a negation, say $M = N \yields \fff$ holds only if there is no (respectful) substitution unifying $M$ and $N$ (otherwise for some respectful $\sigma$, $M\sigma = N\sigma$, but $\fff\sigma$ can never hold).

Like implication, modalities are assumed to hold in every accessible world.
For the diamond modality the ``all reachable worlds'' proviso is redundant, since no respectful substitution or extra name distinction can disable a transition previously enabled.

For example $\match{x \not= y }\tau \not\vDash \diam{\tau}\ttt$, since in the world with no assumptions about $x$ and $y$, 
$\match{x \not= y }\tau$ cannot perform any actions. 
In contrast, $\match{x \not= y }\tau \vDash x \not= y \yields \diam{\tau}\ttt$,
by the following argument.
For all distinctions $\mathcal{D}$ such that $\mathcal{D} \vDash x \not= y$, 
$\match{x \not= y }\tau \vDash^{\mathcal{D}, x^i\cdot y^i} x = y \yields \fff$ holds since there is no substitution $\sigma$ respecting $\mathcal{D}$ such that $x\sigma = y\sigma$.
Furthermore, for all such distinctions, $\match{x \not= y }\tau \vDash^{\mathcal{D}, x^i\cdot y^i} \diam{\tau}\ttt$ holds since $\mathcal{D}, x^i\cdot y^i \colon \match{x \not= y }\tau \lts{\tau} 0$, as required.
In short, the formulae reads ``in all worlds where $x$ and $y$ can never be equated a $\tau$ transition is enabled.'' 


\begin{comment}
\begin{figure}
\[
\begin{array}{lcl}
P \vDash^{h} \ttt && \mbox{always holds.}
\\
P \vDash^{ h} M = M && \mbox{always holds.}
\\
%P \vDash^{h,\mathcal{E}} \boxm{M = M}\phi & \mbox{iff} & P \vDash^{h,\mathcal{E}} \phi.
%\\
%P \vDash^{h,\mathcal{E}} \boxm{M \not= N}\phi & \mbox{iff} & h \vDash M \not= N ~\mbox{and}~ P \vDash^{h,\mathcal{E}} \phi.
%\\
P \vDash^{ h} \phi_1 \land \phi_2 &\mbox{iff}&
  P \vDash^{ h} \phi_1 ~\mbox{and}~ P \vDash^{ h} \phi_2.
\\
P \vDash^{ h} \phi_1 \lor \phi_1 &\mbox{iff}&
  P \vDash^{ h} \phi_1 ~\mbox{or}~ P \vDash^{ h} \phi_2.
\\
P \vDash^{ h} \phi_1 \yields \phi_2 &\mbox{iff}&
%\forall \sigma \respecting h \mbox{and} \vec{x}, \vec{y},
\forall \sigma, \mathcal{D}, ~\mbox{such that}~ \sigma \respects  h,
%,~\mbox{and}~\forall ~\mbox{distinctions}~ \mathcal{D}, 
%\forall ~\mbox{distinctions}~\mathcal{D} ~\mbox{and}~\forall \sigma \respecting \mathcal{D},  h ,
\\
&&  P\sigma \vDash^{\mathcal{D},  h \cdot{\sigma} \phi_1\sigma ~\mbox{implies}~ P\sigma \vDash^{\mathcal{D},  h\sigma} \phi_2\sigma.
\\
%P \vDash^{ h} \phi_1 \yields \phi_2 &\mbox{iff}&
%\forall \sigma \respecting h,
%  P\sigma \vDash^{h\sigma} \phi_1\sigma ~\mbox{implies}~ P\sigma \vDash^{h\sigma} \phi_2\sigma.
%\\
P \vDash^{ h} \diam{\alpha}\phi &\mbox{iff}&
  \exists\,Q,~ P \lts{\alpha} Q ~\mbox{and}~ Q \vDash^{ h} \phi.
\\
P \vDash^{ h} \diam{\co{M}(z)}\phi &\mbox{iff}&
  \exists\,Q,~ P \lts{\co{M}(z)} Q ~\mbox{and}~ Q \vDash^{h \cdot z^o} \phi.
\\
P \vDash^{ h} \diam{{M}(z)}\phi &\mbox{iff}&
  \exists\,Q,~ P \lts{{M}(z)} Q ~\mbox{and}~ Q \vDash^{h \cdot z^i} \phi.
\\
P \vDash^{ h} \boxm{\alpha}\phi &\mbox{iff}&
\forall \sigma, \mathcal{D}, Q ~\mbox{such that}~ \sigma \respects  h,
%\forall \sigma \respecting  h, \forall ~\mbox{distinctions}~ \mathcal{D}, ~\mbox{and}~\forall Q,
%\forall ~\mbox{distinctions}~\mathcal{D} ~\mbox{and}~\forall \sigma \respecting \mathcal{D},  h ,
%  \forall \sigma \respecting h,
\\&&
    \mathcal{D}, h\sigma \colon P\sigma \lts{\alpha\sigma} Q  ~\mbox{implies}~
    Q \vDash^{\mathcal{D}, h\sigma} \phi\sigma.
\\
P \vDash^{ h} \boxm{\co{M}(z)}\phi &\mbox{iff}&
\forall \sigma, \mathcal{D}, Q ~\mbox{such that}~ \sigma \respects  h,
%\forall \sigma \respecting  h, \forall ~\mbox{distinctions}~ \mathcal{D}, ~\mbox{and}~\forall Q,
%\forall ~\mbox{distinctions}~\mathcal{D} ~\mbox{and}~ \forall \sigma \respecting \mathcal{D},  h ,
%  \forall\sigma \respecting h,~ 
\\&&
\mathcal{D}, h\sigma \colon P\sigma \lts{\co{M\sigma}(z)} Q ~\mbox{implies}~ Q \vDash^{\mathcal{D}, h\sigma \cdot z^o} \phi\sigma.
\\
 P \vDash^{ h} \boxm{{M}(z)}\phi &\mbox{iff}&
\forall \sigma, \mathcal{D}, Q ~\mbox{such that}~ \sigma \respects  h,
%\forall \sigma \respecting  h, \forall ~\mbox{distinctions}~ \mathcal{D},  ~\mbox{and}~\forall Q,
%\forall ~\mbox{distinctions}~\mathcal{D} ~\mbox{and}~\forall \sigma \respecting \mathcal{D},  h ,
%  \forall \sigma \respecting h, \forall Q, 
\\&&
    \mathcal{D}, h\sigma \colon P\sigma \lts{M\sigma(z)} Q  ~\mbox{implies}~ Q \vDash^{\mathcal{D}, h\sigma \cdot z^i} \phi\sigma.
\end{array}
\]
\caption{The semantics of intuitionistic modal logic $\mathcal{OM}$. Variable $z$ is assumed to be fresh.}\label{figure:OM}
\end{figure}
\end{comment}

\subsection{Characterisation of open bisimilarity with mismatch using $\mathcal{OM}$}

The logical characterisation of open bisimulation is broken into a soundness and completeness result.
Soundness states that if two processes are open bisimilar
then they satisfy all the same formulae $\mathcal{OM}$.
\begin{theorem}[soundness]
If $P \lsim Q$, then for all $\phi$,
$P \vDash \phi$ if and only if $Q \vDash \phi$.
\end{theorem}
The proof of soundness proceeds by induction over the structure of formulae.

The interesting case is completeness.
The contrapositive of completeness states:
if two processes are not open bisimilar, then there is some formula that holds for one process but not the other process. For calculi such as the finite $\pi$-calculus with mismatch where open bisimulation is decidable, proving the contrapositive argument is sufficient to establish completeness.
\begin{theorem}[completeness]
If, for all $\phi$,
$P \vDash \phi$ if and only if $Q \vDash \phi$,
then $P \lsim Q$.
\end{theorem}
The main proof in this work is therefore to prove the contrapositive to the above theorem.
For this some auxiliary results are required presented next.


\subsection{Preliminaries}

We require a direct definition of ``non-bisimilarity'' that holds whenever there is a distinguishing strategy for an open bisimulation game.
Bisimulation is defined co-inductively; hence its dual definition ``non-bisimilarity'' is defined inductively. 
\begin{definition}[non-bisimilarity]\label{def:non-bisim}
Inductively define the family of relations $\not\sim^{h}_n$, for $n \in \mathbb{N}$.
%The base case $\not\sim^{h}_0$ is when, in some world $h$ player $P$ can make a move, that cannot be matched by the other player $Q$ in the same world.
%, without stronger assumptions.
%The class of all such pairs of processes form the base relation  for the construction of the non-bisimilarity relation, say $P \not\sim^h_0 Q$.
The base relation $\not\sim^{h}_0$ is the least symmetric relation
such that for any $P$ and $Q$, $P \not\sim^{h}_0 Q$ whenever there exist process $P'$, action $\pi$, substitution $\sigma$ respecting $h$, and distinction $\mathcal{D}$, such that:
$\mathcal{D},h\sigma \colon P\sigma \lts{\pi\sigma} P'$, for $x \in \bn{\pi}$, $x$ is fresh for $P\sigma$, $Q\sigma$ and $h\sigma$, and there is no $Q'$ such that $\mathcal{D},h\sigma \colon Q\sigma \lts{\pi\sigma} Q'$.

Inductively, $\not\sim_{n+1}^{h}$ is the least symmetric relation extending $\not\sim_{n}^{h}$ such that 
$P \not\sim^{h}_{n+1} Q$ whenever 
for some substitution $\sigma$ respecting $h$, and distinction $\mathcal{D}$ one of the following holds:
\vspace*{-1.5ex}
\begin{itemize}
\item $\mathcal{D},h\sigma \colon P\sigma \lts{\alpha\sigma} P'$ and, for all $Q_i$ such that $\mathcal{D},h\sigma \colon Q\sigma \lts{\alpha} Q_i$, we have $P' \not\sim^{h\sigma}_n Q_i$, where $\alpha$ is $\tau$ or $\co{M}N$.
\item $\mathcal{D},h\sigma \colon P\sigma \lts{\co{a\sigma}(x)} P'$, and, for all $Q_i$ and $x$ fresh for $P\sigma$, $Q\sigma$ and $\mathcal{D},h\sigma$, such that $\mathcal{D},h\sigma \colon Q\sigma \lts{\co{a\sigma}(x)} Q_i$, we have $P' \not\sim^{h\sigma \cdot x^o}_n Q_i$.
\item $\mathcal{D},h\sigma \colon P\sigma \lts{a\sigma(x)} P'$, and for all $Q_i$ and $x$ fresh for $P\sigma$, $Q\sigma$ and $\mathcal{D},h\sigma$, such that $\mathcal{D},h\sigma \colon Q\sigma \lts{a\sigma(x)} Q_i$, we have $P' \not\sim^{h\sigma \cdot x^i}_n Q_i$.
\vspace*{-1.2ex}
\end{itemize}
The relation $\not\sim^{h}$, pronounced non-bisimilarity with history $h$, is defined to be the least relation containing $\not\sim^{h}_n$ for all $n \in \mathbb{N}$,
i.e.\ $\bigcup_{n\in\mathbb{N}} \not\sim^{h}_n$.
Similarly to open bisimulation, $P \not\sim Q$ is defined as $P \not\sim^{x_1^i\cdot\hdots x_m^i} Q$ where $\fv{P}\cup\fv{Q} \subseteq \left\{ x_1, \hdots x_m \right\}$.
	\\[-1.5ex]
\end{definition}

In the definition above each stratum, indexed by $n$, contains all pairs of processes that can be distinguished by a strategy with depth at most $n$, i.e.,\ at most $n$ transitions are required to reach a pair of processes and world in which a process can make a move that the other process cannot match.



We require the following terminology for substitutions,
and abbreviations for formulae.
\begin{definition}
Composition of substitutions $\sigma$ and $\theta$ is defined such that $P \big(\sigma \cdot \theta\big) = \big(P \sigma\big) \theta$, for all processes $P$.
For substitutions $\sigma$ and $\theta$,
$\sigma \leq \theta$ whenever there exists $\sigma'$ such that $\sigma \cdot \sigma' = \theta$.
For distinctions, $\mathcal{E} \leq \mathcal{D}$ whenever for all $x \not= y \in \mathcal{E}$,
$\mathcal{D} \vDash x \not= y$.

For substitution $\sigma$ and distinction $\mathcal{D}$, represented respectively as $\sub{x_1}{y_1}\cdots\,\sub{x_n}{y_n}$ and $\left\{ w_1 \not= z_1, \hdots w_m \not= z_m \right\}$ we have the following abbreviations:
\begin{itemize}
\item $\boxm{\sigma, \mathcal{D}}\phi$ abbreviates $x_n=y_n \wedge \hdots \wedge  x_1=y_1 \wedge w_1 \not= z_1 \wedge  \hdots \wedge w_m \not= z_m \yields \phi$;
\item $\diam{\sigma, \mathcal{D}}\phi$ abbreviates $x_n=y_n \wedge \hdots \wedge  x_1=y_1 \wedge w_1 \not= z_1 \wedge  \hdots \wedge w_m \not= z_m \wedge \phi$.
\end{itemize}
%For a finite substitution $\sigma$ the formula $\boxm{\sigma}\phi$ abbreviates any formula $[x_1=z_1]\hdots[x_n=z_n]\phi$ such that for all $x$ and $z$, $x\sigma = z\sigma$ if and only if $x = z$ is in the least equivalence relation generated by $\left\{ x_1 = z_1 , \hdots x_n = z_n \right\}$.
For finite set of formulae $\phi_i$, $\bigvee_i \phi_i$ abbreviates $\phi_1 \vee \!\hdots\! \vee \phi_n$, where the empty disjunction is $\fff$.
Similarly $\bigwedge_i \phi_i$ abbreviates $\phi_1 \wedge \hdots \wedge \phi_n$, where the empty conjunction is $\ttt$.
\end{definition}

We require the following technical lemmas.
%The first ensures there are finitely many equalities between variables characterising all substitutions that enable a transition.
The first, image finiteness, ensures that in every ``world'' there are finitely many reachable states in one step, up to renaming.
The second is a useful property that follows by induction from the definitions.
The third is required in inductive cases involving bound output and input.
The fourth is a monotonicity property for satisfaction.
The fifth is a monotonicity property for transitions ensuring names bound by label are not changed by a substitution.
%\begin{lemma}\label{lemma:sub}
%For all $P$ and $\pi$ there exist finitely many $\sigma_j$ and $Q_j$ such that 
%for all $\sigma$, if $P\sigma \lts{\pi\sigma} Q$, then there exist $j$ and $\theta$ such that $\sigma_j\cdot\theta = \sigma$, $Q_j\theta = Q$ and $P\sigma_j \lts{\pi\sigma_j} Q_j$.
%\ross{Still not completely this is the right lemma. Probably OK, but will think again.} 
%\end{lemma}
\begin{lemma}\label{lemma:finite}
For process $P$, action $\pi$,
history $h$ and distinction $\mathcal{E}$,
there are finitely many $P_i$ such that $h \colon P \lts{\pi} P_i$.
%up to $\alpha$-conversion.
\end{lemma}
\begin{lemma}
\label{lemma:box}
If for all $\mathcal{E} \leq \mathcal{D}$
and $\theta$ respecting $\mathcal{D}, h$,
such that $\sigma \leq \theta$, we have $P\theta \vDash^{\mathcal{D}\theta,h\theta} \phi\theta$,
then $P \vDash^{h} \boxm{\sigma,\mathcal{E}}\phi$ holds.
\end{lemma}
\begin{lemma}\label{lemma:respects}
If $\sigma \cdot \theta$ respects $\mathcal{D}, h$,
then $\theta$ respects $\mathcal{D}\sigma, h\sigma$.
\end{lemma}
\begin{lemma}\label{lemma:mono}
If $P \vDash^{h} \phi$ holds then $P\theta \vDash^{\mathcal{E}\theta,h\theta} \phi\theta$ holds
for any $\theta$ respecting $h$.
\end{lemma}
\begin{lemma}\label{lemma:mono-trans}
If $ h \colon P \lts{\pi} Q$ then $ h \colon P\theta \lts{\pi\theta} Q\theta$,
for all $\theta$ respecting $ h$ such that if $x \in \bn{\pi}$ and $x\theta = x$.
%	\\[-1.5ex]
\end{lemma}

\subsection{Algorithm for distinguishing formulae}
The constructive definition of non-bisimilarity gives a tree of substitutions and actions forming a strategy showing that two processes are not open bisimilar.
The following proposition shows that \OM\ formulae are sufficient to capture such strategies.
For any strategy that distinguishes two processes, we can construct \textit{distinguishing} \OM\ formulae.
A distinguishing formula holds for one process but not for the other process.
Furthermore, % according to the construction in the proof below,
there are always at least two distinguishing formulae,
one biased to the left and another biased to the right,
as in the construction of the proof for the following proposition.
As discussed in the introduction, the left bias cannot be simply
obtained by negating the right bias and vice versa; both must be constructed simultaneously and
may be unrelated by negation.
\begin{proposition}[distinguishing formulae]\label{proposition:non-bisim}
If $P \not\sim Q$ then there exists $\phi_L$ such that $P \vDash \phi_L$ and $Q \not\vDash \phi_L$, and also 
there exists $\phi_R$ such that $Q \vDash \phi_R$ and $P \not\vDash \phi_R$.
\end{proposition}




\subsection{Examples of distinguishing formulae involving mismatch}

Since the proof of completeness is constructive, an algorithm can be extracted from the proof that generates distinguishing formulae for each pair of processes that are not open bisimilar.
We illustrate this algorithm on examples of distinguished processes.

\paragraph{Example requiring intuitionistic assumptions.}
Processes $0$ and $\match{x \not= y}.\tau$ are distinguished, since the later can perform a $\tau$ action in a ``world'' where $x \not= y$, but the $0$ can never perform a $\tau$ transition.
This is a base case of the algorithm, yielding distinguishing formulae 
$0 \vDash \boxm{\tau}\fff$ and $\match{x \not= y}.\tau \vDash x \not= y \yields \diam{\tau}\ttt$.

Processes $\tau$ and $\match{x \not= y}.\tau$ are also distinguished, 
since $\tau$ can always perform a $\tau$ transition, but $\match{x \not= y}.\tau$ can only perform a $\tau$ transition in worlds where $x \not= y$. 
This is also a base case of the algorithm, yielding distinguishing formulae
$\tau \vDash \diam{\tau}\ttt$ and $\match{x \not= y}.\tau \vDash \boxm{\tau}\left( x \not= y \right)$.

As variation of a classic example consider:
$
\tau + \tau.\tau
\not\sim 
\tau + \tau.\tau + \tau\match{x \not= y}.\tau
$.
The later process can perform a $\tau$ transition to reach process
$\match{x \not= y}.\tau$. However, the former process can only reach $0$ or $\tau$ by a $\tau$ transition. As noted above neither $0$ not $\tau$ is open bisimilar to $\match{x \not= y}.\tau$. Hence by applying the inductive case of the algorithm, we can construct the following formulae from the conjunction and disjunction of the appropriate distinguishing formulae constructed above:
\[
\tau + \tau.\tau \vDash \boxm{\tau}\left(\boxm{\tau}\fff \vee \diam{\tau}\ttt\right)
\]
\[
\tau + \tau.\tau + \tau\match{x \not= y}.\tau
\vDash
\diam{\tau}.\left(  \left(x \not= y \yields \diam{\tau}\ttt\right) \wedge \boxm{\tau}\left( x \not= y \right) \right)
\]
Notably if we exchange the above two processes and formulae, satisfiability would still hold under classical assumption. Thus the above example depends on interpreting $\mathcal{OM}$ in an intuitionistic meta-framework.

\paragraph{Example involving outputs.}
Observe that $\match{z \not= y}\tau \not\sim^{x^i \cdot z^o \cdot y^i} \tau$.
For history $x^i \cdot z^o \cdot y^i$, it is not inevitable that $\match{z \not= y}\tau$ performs a $\tau$ transition since $\sub{y}{z}$ respects $x^i \cdot z^o \cdot y^i$.
Thus a distinguishing formulae are $
\match{z \not= y}\tau \vDash^{x^i \cdot z^o \cdot y^i} \boxm{\tau}(z \not= y)$ and
$\tau \vDash^{x^i \cdot z^o \cdot y^i} \diam{\tau}$ respectively.
Observe that the histories are recorded in the satisfaction relation.

Now consider the following processes are not open bisimilar.
\[
\nu z.\cout{x}z.x(y).\match{z \not= y}\tau
\not\sim 
\nu z.\cout{x}z.x(y).\tau
\]
Both processes can perform the actions $\co{x}(z)$ and $x(y)$, to reach the above pair of processes $\match{z \not= y}\tau \not\sim^{x^i \cdot z^o \cdot y^i} \tau$.
Thus, by applying the inductive case of the algorithm twice, the following distinguishing formulae can be constructed.
\[
\nu z.\cout{x}z.x(y).\match{z \not= y}\tau \vDash \boxm{\co{x}(z)}\boxm{x(y)}\boxm{\tau}(z \not= y)
\]
\[
\nu z.\cout{x}z.x(y).\tau \vDash \diam{\co{x}(z)}\diam{x(y)}\diam{\tau}
\]




%However, by inducing mismatch $z \not= y$, we observe that $\match{z \not= y}\tau \not\sim^{z \not= y, x^i \cdot z^o \cdot y^i} 0$, since $z \not= y, x^i \cdot z^o \cdot y^i \colon \match{z \not= y}\tau \lts{\tau} 0$, but $0$ remains deadlocked in any context.


\begin{comment}
For processes $\nu n.\co{a}n.\match{a \not= n}\tau \lsim^{a^i} \nu n.\co{a}n.\tau$

\[
\nu a. \co{c}{a}.c(y).\match{a \not= y}\tau \not\sim \nu a.\co{c}a.c(y)
\]
\begin{proof}
\[
\nu a. \left( \sub{u}{a} \cpar \match{u \not= y}\tau\right)
\not\lsim^{c^i\cdot u^o \cdot y^i, u \not= y}
\nu a. \left( \sub{u}{a} \cpar 0\right)
\]
Since
\[
\begin{prooftree}
\begin{prooftree}
\begin{prooftree}
c^i\cdot u^o \cdot y^i \cdot a^o, u \not= y
\vDash 
\tau
\lts{\tau}
0
\quad
c^i\cdot u^o \cdot y^i \cdot a^o, u \not= y \vDash \match{u \not= y}
\justifies
c^i\cdot u^o \cdot y^i \cdot a^o, u \not= y
\vDash 
\match{u \not= y}\tau
\lts{\tau}
0
\end{prooftree}
\justifies
c^i\cdot u^o \cdot y^i \cdot a^o, u \not= y
\vDash 
\sub{u}{a} \cpar \match{u \not= y}\tau
\lts{\tau}
\sub{u}{a} \cpar 0
\end{prooftree}
\justifies
c^i\cdot u^o \cdot y^i, u \not= y
\vDash 
\nu a. \left( \sub{u}{a} \cpar \match{u \not= y}\tau\right)
\lts{\tau}
\nu a. \left( \sub{u}{a} \cpar 0\right)
\end{prooftree}
\]
but 
$\nu a. \left( \sub{u}{a} \cpar 0\right)$
can perform no action in any world.

The non bisimulation strategy follows since.
\[
\nu a. \co{c}{a}.c(y).\match{a \not= y}\tau
\lts{\co{c}(u)}
\nu a. \left( \sub{u}{a} \cpar c(y).\match{a \not= y}\tau\right)
\lts{{c}(y)}
\nu a. \left( \sub{u}{a} \cpar \match{a \not= y}\tau\right)
\]
and
\[
\nu a. \co{c}{a}.c(y)
\lts{\co{c}(u)}
\nu a. \left( \sub{u}{a} \cpar c(y) \right)
\lts{{c}(y)}
\nu a. \left( \sub{u}{a} \cpar 0 \right)
\]
\qed
\end{proof}

Not open bisimilar:
\[
\nu a.\co{c}a.c(y).\match{a \not= y}\tau
\not\sim 
\nu a.\co{c}a.c(y)
\]
Biased to left:
\[
\nu a.\co{c}a.c(y).\match{a \not= y}\tau
\vDash
\diam{\co{c}(u)}\diam{c(y)}\left( \left(u = y \yields \fff\right) \yields \diam{\tau}\ttt\right)
\]
Biased to right:
\[
\nu a.\co{c}a.c(y)
\vDash
\boxm{\co{c}(u)}\boxm{c(y)}\boxm{\tau}\fff
\]
\end{comment}


==> piopen.tex <==
\section{Open bisimulation with mismatch}

This section introduces a conservative extension of open bisimulation that can handle mismatch.
The significant change is an additional clause that induces inequalities.

In the standard definition of open bisimulation, we consider every transition enabled under any substitution. For example, $\left(\match{x = y}\tau\right)\sub{x}{y} \lts{\tau} 0$, hence $\match{x = y}\tau$ is distinguished from $0$ which remains deadlocked under the substitution.
Closing by substitutions has the effect of inducing name equalities during state space exploration.

The additional clause can be used to generate additional fresh names (retrospectively).
These fresh names allowing mismatches to be resolved by the labelled transition system. 
For example, 
given history $x^i\cdot y^i$, process $\match{x \not= y}\tau$ cannot act;
however extending with fresh name in place of $x$ we obtain $x^i\cdot y^i \cdot z^o \colon \match{z \not= y}\tau \lts{\tau} 0$.
In this way, $\match{x \not= y}\tau$ is distinguished from $0$.
%We can see the equalities and inequalities induced to be the ``world'' reachable from each state.
The first bullet point in the following definition induces (respectful) equalities; while the second is used to induce inequalities.
\begin{definition}[open bisimulation]\label{def:open}
A symmetric relation indexed by an environment $\mathrel{\mathcal{R}}$ is an open bisimulation whenever,
if $P \mathrel{\mathcal{R}}^{h} Q$ the following hold:
\begin{itemize}
\item If $\sigma$ respects $h$, then $P\sigma \mathrel{\mathcal{R}}^{h\sigma} Q\sigma$.
%\item If $x$ and $y$ are distinct variables, then $P \mathrel{\mathcal{R}}^{x \not= y, h} Q$.
\item For $x$ fresh for $P$, $Q$ and $h$, and for any $z$, we have $P\sub{z}{x} \mathrel{\mathcal{R}}^{h \cdot x^o} Q\sub{z}{x}$.
\item If $P \lts{\alpha} P'$ then there exists $Q'$ such that $Q \lts{\alpha} Q'$ and $P' \mathrel{\mathcal{R}}^{ h} Q'$, where $\alpha$ is of the form $\tau$ or $\co{M}N$.
\item If $P \lts{M(x)} Q'$, where $x$ fresh for $P$, $Q$ and $h$, then there exists $Q'$ such that $Q \lts{M(x)} Q'$ and $P' \mathrel{\mathcal{R}}^{ h\cdot x^i} Q'$.
\item If $P \lts{\co{M}(x)} P'$, where $x$ fresh for $P$, $Q$ and $h$, then there exists $Q'$ such that $Q \lts{\co{M}(x)} Q'$ and $P' \mathrel{\mathcal{R}}^{ h\cdot x^o} Q'$.
\end{itemize}
Open bisimilarity $\lsim$ is defined such that $P \lsim Q$ holds whenever there exists open bisimulation $\mathcal{R}$
such that $P \mathrel\mathcal{R}^{x^i_1 \cdot x^i_2 \cdot \hdots x^i_n} Q$ holds, where $\fv{P} \cup \fv{Q} \subseteq \left\{ x_1, x_2, \hdots , x_n \right\}$.
\end{definition}

The above definition is mostly standard
other than the clause inducing distinctions and the extra environment information for labelled transitions. At any point, a labelled transitions enabled for a process, must be matched by a transition with the same label by the other process. 
Input transition update the history with a fresh input variable, while bound outputs update the history with a fresh private name.

\begin{comment}
For compositionality, it is essential not to allow a process such as $\match{x \not= y}\tau$ to always make progress. To see why, observe that the following processes are not open bisimilar according to our definition.
\[
\xymatrix{
a(x).\tau + a(x).\match{x \not= y}\tau
\ar^{a(x)}[d]
&
\not\sim
&
a(x).\match{x \not= y}\tau
\ar^{a(x)}[d]
\\
\tau
&
\not\sim
&
\match{x \not= y}\tau
}
\]
The processes $\tau$ and $\match{x \not= y}\tau$ are distinguished, since $\tau$ can always act, but $\match{x \not= y}\tau$ may only make a transition in a context with name distinction $x \not= y$.

It can be tempting to \textbf{na{\"i}vely} assume that $\match{x \not= y}\tau$ can always perform a $\tau$ action. This assumption has been frequently made in the literature, since classical definitions of bisimulation assume terms are closed (i.e.\ $\pi$-calculus names are constants).
However, collapsing these processes, would collapse the processes in the above example.
This would break compositionality since in the context $\co{a}y \cpar \left\{ \cdot \right\}$ the process $a(x).\match{x \not= y}\tau$ can only perform one input action, but the process $a(x).\tau + a(x).\match{x \not= y}\tau$ can perform an input followed by a $\tau$ transition.
\end{comment}

\paragraph{Examples of open bisimilar processes.}
The following processes are open bisimilar.
\[
\nu z.\co{x}z.\match{x \not= z}\tau
\sim
\nu z.\co{x}z.\tau
\]
Observe that $\nu z.\co{x}z.\match{x \not= z}\tau \lts{\co{x}(z)} \match{x \not= z}\tau$
and $\nu z.\co{x}z.\tau \lts{\co{x}(z)} \tau$,
accumulating history $x^i \cdot z^o$. Now, since $x^i \cdot z^o \vDash x \not= z$, automatically $x^i \cdot z^o \colon \match{x \not= z}\tau \lts{\tau} 0$, without any further assumptions, hence $\match{x \not= z}\tau \sim^{x^i \cdot z^o} \tau$.

Similarly, the following processes are also open bisimilar:
$\nu z.\match{z \not= y}\tau
\lsim
\tau$.
As discussed in the previous section, $x^i \colon \nu z.\match{z \not= y}\tau \lts{\tau} 0$
without further assumptions.

\begin{comment} Flawed example.
The following processes are also open bisimilar.
\[
\nu z. \co{x}{z}.x(y).\match{z \not= y}\tau \not\sim \nu z.\co{x}z.x(y).\tau
\]
Both processes can perform actions $\co{x}(z)$ and $x(y)$, accumulating the history $x^i \cdot z^o \cdot y^i$. Furthermore, $x^i \cdot z^o \cdot y^i \colon \match{z \not= y}\tau \lts{\tau} 0$, since there is no substitution $\sigma$ respecting $x^i \cdot z^o \cdot y^i$ such that $z\sigma = y\sigma$. Hence $\match{z \not= y}\tau \sim^{x^i \cdot z^o \cdot y^i} 0$.
\end{comment}

Clearly $\match{x \not= z}\left( \co{x}y \cpar z(w) \right) \sim 
\match{x \not= z}\left(\co{x}y.z(w) + z(w).\co{x}y\right)$ holds.
This can be established directly; or by property $\co{x}y \cpar z(w) \sim \co{x}y.z(w) + z(w).\co{x}y + \match{x = z}\tau$ combined with $\match{x \not= y}(P + Q) \sim \match{x \not= y}P + \match{x \not= y}Q$ and
$\match{x = y}\match{x \not= y}P \sim 0$.

Consider $\match{x \not= z}\co{x}y \cpar z(w)$ and $\match{x \not= z}\left(\co{x}y \cpar z(w)\right)$. Although the send and receive actions cannot interact, these processes are not open bisimilar. The former can always perform action $z(w)$, even if $x$ and $z$ are equated by the context; but the later can only perform action $z(w)$ in a context where $x$ and $y$ are guaranteed to be distinct.



\subsection{Soundness with respect to established notions of bisimulation}

An essential property is that open bisimilarity is preserved by any context.
For example, if open bisimulation \textbf{wrongly} equates $\match{x \not= y}\tau$ and $\tau$, then it would not be a congruence since context $z(x).\left\{\ \cdot\ \right\} \cpar \co{z}y$ distinguishes these processes.
Fortunately, having the insight to treat mismatches between variables intuitionistically avoids this problem (or, more generally, mismatches between open messages). 
\begin{theorem}\label{theorem:congruence}
Open bisimilarity is a congruence.
\end{theorem}



A barb represents the ability to observe an input or output action on a channel $M$.
\begin{definition}[barb]
A process $P$ has barb $M$, written $\barb{P}{M}$,
whenever there exists process $Q$ 
such that $P \lts{\co{M} N} Q$,
or $P \lts{\co{M} (x)} Q$,
or $P \lts{M (x)} Q$.
\end{definition}

Barbs are typically used to defined a notion called \textit{barbed congruence}~\cite{Milner1992}.
However, in the context of open bisimilarity a tighter reference is \textit{open barbed bisimilarity}~\cite{Sangiorgi2001}.
Open barbed bisimulation differs from barbed bisimulation since it closes by all contexts at every $\tau$ transition.
\begin{definition}[open barbed bisimulation]\label{def:open-barbed}
An open barbed bisimulation $\rel$ is a symmetric relation over processes
such that whenever $P \rel Q$ holds 
the following hold:
\begin{itemize}
\item For all contexts $\context{}$, $\context{P} \rel \context{Q}$.
\item If $\barb{P}{M}$ then $\barb{Q}{M}$.
\item If $P \lts{\tau} P'$, there exists $Q'$ such that $Q \lts{\tau} Q'$ and $P' \rel Q'$ holds.
\end{itemize}
Open barbed bisimilarity is defined to be the greatest open barbed bisimulation.
\end{definition}
We have that, as a consequence of Theorem~\ref{theorem:congruence},
that open bisimulation is sound with respect to open barbed bisimilarity (and hence barbed congruence).
\begin{corollary}\label{corollary:openbarbed}
Open bisimilarity is sound with respect to open barbed bisimilarity.
\end{corollary}

Even without mismatch~\cite{Sangiorgi2001}, the converse to Corollary~\ref{corollary:openbarbed} does not hold.
None-the-less, the contrapositive of Corollary~\ref{corollary:openbarbed} can be useful for explaining why some processes are not open bisimilar.
Consider the example from the introduction: $\tau \not\sim \match{x=y}\tau + \match{x\not=y}\tau$.
In the empty context, the former can perform a $\tau$ transition but the latter cannot perform any action. 
Hence the processes are not open barbed bisimilar and hence not open bisimilar.
Note, for the branch with mismatch to trigger, we are required to close with a context such as $\nu y.\left\{\ \cdot\ \right\}$ that forces inequality $x\not=y$.

Open bisimulation can be seen as a reconciliation between open barbed bisimulation and strong equivalence, in the sense that it is sound with respect to both.
In the following we assume the long established definition strong equivalence --- the greatest congruence contained in late bisimilarity. Late bisimulations immediately cater for mismatch~\cite{Parrow1995} since all messages are closed terms, and hence names are treated as constants.
\begin{proposition}\label{proposition:late}
Open bisimilarity is sound with respect to strong equivalence for $\pi$-calculus with mismatch.
\end{proposition}
The proof works by constructing a late bisimulation from any open bisimulation.
The trick is to assume a sufficiently large supply of extruded private names to ground processes after every input transition. 
The above proposition relies on the 
fact that, assuming all free variables appear as private outputs in the history,
the labelled transitions in Fig.~\ref{figure:pi} coincides with classical $\pi$-calculus labelled transition system~\cite{Parrow1995}.
For example, $x^o \cdot y^o \colon \match{x \not= y}\tau \lts{\tau} 0$,
since $x$ and $y$ can never be unified given history $x^o \cdot y^o$.
More details are provided when we extend late bisimilarity to the applied $\pi$-calculus later in this paper.

\begin{comment}
\begin{definition}[late bisimulation]
A symmetric relation $\mathrel{\mathcal{R}}$ is a late bisimulation whenever,
if $P \mathrel{\mathcal{R}} Q$, then:
\begin{itemize}
\item If $P \lts{\alpha} P'$ then there exists $Q'$ such that $Q \lts{\alpha} Q'$ and $P' \mathrel{\mathcal{R}} Q'$, where $\alpha$ is of the form $\tau$ or $\co{M}N$.
\item If $P \lts{M(x)} Q'$, where $x$ fresh for $P$ and $Q$, then there exists $Q'$ such that $Q \lts{M(x)} Q'$ and 
for all messages $N$, $P'\sub{x}{N} \mathrel{\mathcal{R}} Q'\sub{x}{N}$.
\item If $P \lts{\co{M}(x)} P'$, where $x$ fresh for $P$ and $Q$, then there exists $Q'$ such that $Q \lts{\co{M}(x)} Q'$ and $P' \mathrel{\mathcal{R}} Q'$.
\end{itemize}
Late bisimilarity is the greatest late bisimulation.
Late congruence is the greatest congruence contained in late bisimilarity.
\end{definition}
\end{comment}


As a sanity check observe Definition~\ref{def:open} is conservative with respect to established definitions of open bisimulation without mismatch~\cite{sangiorgi96acta}.
\begin{proposition}[conservativity]
For processes $P$ and $Q$ without mismatch,
$P \sim Q$ iff $P$ and $Q$ are open bisimilar according to the original definition of open bisimulation.
\end{proposition}
To see why the above hold observe, for processes without mismatch: firstly, the labelled transition systems coincide; and, secondly, the additional clause inducing inequalities cannot disable any transition that was previously enabled.






==> popl_reviews <==
Dear author,

The The 46th ACM SIGPLAN Symposium on Principles of Programming Languages
(POPL 2019) program committee is sorry to inform you that your submission
#37 was rejected, and will not appear in the conference.

       Title: A Bisimilarity Congruence for the Applied pi-Calculus
              Sufficiently Coarse to Verify Privacy Properties
     Authors: Ross Horne (Nanyang Technological University)
        Site: https://popl19.hotcrp.com/paper/37?cap=037a9phsUADm0Xc

Reviews and comments on your paper are appended to this email. Note that
your
reviews may have changed due to the discussion during the PC meeting. This
discussion has been summarized in a brief comment at the end of this
message.
The submissions site also has the paper's reviews and comments, as well as
more information about review scores.

Contact Stephanie Weirich <sweirich@cis.upenn.edu> with any questions or
concerns.

- POPL 2019 Submissions

Review #37A
===========================================================================

Overall merit
-------------
C. Weak reject

Reviewer expertise
------------------
Z. No familiarity

Paper summary
-------------
I'm not quite sure what the contributions of this paper are. I think
that the main technical contributions are definitions of (strong or
weak) quasi-open bisimilarity for a calculus called the applied
π-calculus, along with proofs that these notions of bisimilarity are
sound and complete with respect to (strong or weak) open barbed
bisimilarity. The paper also includes a modal logic which can be used
to prove that processes are not strong quasi-open bisimilar. I think
the applied π-calculus is also presented in a new way (but there is no
proof of equivalence with the old way; it is stated that the old
presentations did not permit strong notions of bisimilarity).

It seems as if quasi-open bisimilarity has already been investigated
for the π-calculus and something called the π-calculus with mismatch.
As I am not familiar with previous work in this area I don't know
whether the results of this paper are important or just minor variants
of previous results. The presentation suggests that the results are
incremental.

The paper includes several examples motivating the presented calculus
and notions of bisimilarity, but I had trouble following them. Perhaps
the paper's target audience is too small. I would have liked to see an
explanation of the basics of how calculi like the π-calculus are used
to model problems in security and privacy (which seems to be the main
focus of the work). The paper is self-contained in the sense that it
includes a definition of the applied π-calculus (syntax + transition
rules + several notions of bisimilarity). However, the transition
rules of the applied π-calculus are somewhat different from the usual
presentation of the regular π-calculus, and it wasn't obvious to me
that the applied π-calculus models something useful.

I think I found a bunch of mistakes in the text, and after a while I
decided to stop checking every detail. The paper includes some long
proofs, and I did not check them at all. I think work of this kind
(incremental work with lots of subtle, technical details) really
should be supported by machine-checked proofs, to increase the
confidence in the results, and to make life easier for reviewers and
readers.

Strengths
---------
* The results seem useful, assuming that the calculus is useful and
  that the proofs are correct.

Weaknesses
----------
* Presentation targeted at a narrow audience.

* Incremental?

* No machine-checked proofs.

Comments for author
-------------------
Line 135, "the attacker can determine that the server responds to
stimulus pk(k)": What does this mean? The variable k is not in scope.

Figure 2: There is no rule for νx.P, only νx.A.

Figure 2, rule Alias: How is σ ∥ A defined? Is it always well-defined?

Figure 2, last two rules: Please discuss why it is fine to stick to
substitutions {N/x}, rather than substitutions σ with x ∈ dom(σ).

Figure 2, last rule: Why does the last antecedent contain z⃗ rather
than {x} ∪ z⃗ (like in the previous rule)?

Line 274: In should be Inp.

Line 296, "the private name k": Do you mean "n"?

Line 305, "assuming adec(aenc(n, k), pk(k)) =E n": Don't you mean
"adec(aenc(n, pk(k)), k) =E n"? The latter equality follows from the
rules in Figure 1, there is no need to "assume" it.

Line 306: Does ν bind tighter than ∥?

Line 324, "processes": Do you mean "extended processes in normal
form"? If not, then line 327 does not make sense.

"Furthermore, objectively, open barbed bisimilarity is the coarsest
bisimilarity congruence, in the sense that it is by definition a
congruence, and defined independently of the content of the messages
sent and received": I don't follow this argument. How do you define
what a "bisimilarity" is?

"open barbed bisimilarity applies to any language": Any language
defined using a labelled transition system with labels of a certain
kind?

Definition 3.1, "Assuming dom(σ) ∩ x⃗ = ∅ and dom(θ) ∩ y⃗ = ∅": Doesn't
this follow from your statement on lines 197-199?

"This assumption about asymmetric encryption avoids common problems,
including Bleichenbacher's vulnerability on SSL [Bleichenbacher
1998]": In what sense are the problems avoided? Do you mean that your
calculus cannot model the problems? Is this a feature or a bug?

Line 394, "recipe fst(adec(x₃,x₄)) = t": Do you mean "the two recipes
fst(adec(x₃,x₄)) and t"?

Line 401: What does νz⃗.(ρ∥Aσρ) mean? The definition on line 204 does
not cover this case.

Line 404: Is the idea that τ is a process that makes a silent
transition to some process (maybe 0)?

"The freshness assumption for the substitution ensures the same
substitution cannot be applied to extended process
νx.({h(x)/u} ∥ [z = h(x)]τ)": The freshness assumption is that
{h(x)/z} is fresh for dom({h(x)/u}) = {u}, which seems to hold.

Line 410: The reduct should be νx.({x/u} ∥ [x = x]τ), right? A similar
comment applies to the following line.

Line 420, "Notice in a sense the definition is simpler than for the
π-calculus": Do you mean "the π-calculus with mismatch"? And do you
expect that your readers know this definition? I don't.

Line 434: Shouldn't ⟨z,y⟩ be ⟨⟨z,y⟩⟩?

Line 445: Please use the same variable names as above.

Line 459: The processes are not statically equivalent, as witnessed by
the recipes aenc(x,z) and v. Or have I misunderstood something?

Line 470, "least open relation": Do you mean "least open symmetric
relation"?

Line 470, "for all y": And all variables u fresh for {a, k, r} and all
variables v fresh for {a, k, r, u}?

You state that "Critically, message y ranges over all permitted
inputs". Is this correct? The process a(x).P accepts arbitrary inputs
N, with N substituted for x in P. The extended process
{pk(k)/u} ∥ a(x).P also accepts arbitrary inputs N, with N{pk(k)/u}
substituted for x in P. The extended process
νk.νr.({pk(k)/u} ∥ a(x).P) accepts arbitrary inputs N satisfying
k, r ∉ n(N), with N{pk(k)/u} substituted for x in P. You stated that y
should be fresh for {k, r, v}, but (unless I'm mistaken) it could
contain v, and it could contain pk(k).

Line 480, "Observe the branch sending an encrypted message is
enabled": What do you mean? The caption for Figure 2 states that "The
equational theory over message terms can be applied to equate the
occurrences of M in […] Mat", but there is no hint that the
substitution {pk(k)/u} can be applied to [u = pk(k)].

Line 484, "If y is any other term then we have k, r ⊨ y ≠ pk(k)": As I
wrote above y could be pk(k). It could also be, say,
fst(⟨pk(k),true⟩). Perhaps you could prove that, if y =E pk(k) does
not hold, then k, r ⊨ y ≠ pk(k) holds.

Line 475: There is a transition νk.νr.({pk(k)/u} ∥ a̅⟨r⟩) →^{a̅(m)}
νk.νr.({pk(k),r/u,m} ∥ 0) (assuming that m ∉ {k, u}). It seems to me
as if the right-hand side cannot respond to this when y =E pk(k) (with
this particular definition of 𝓢). Similar comments might apply to the
previous two lines.

Line 486: How do you prove that the two extended processes are
statically equivalent? By induction over all pairs of messages?

For the "Example of privacy property", how does the fact that 𝓢 is
defined to be open affect the proof showing that 𝓢 is a quasi-open
bisimulation? Please include some details.

Lemma 3.5, "only if": Do you mean "if"? The last occurrence of P
should presumably be R.

Line 525, "contained in": Do you mean "containing"?

At this point I decided to stop checking details carefully, because,
if the remaining text should have the same density of (perceived)
problems as the preceding text, then this would take far too much
time. I recommend that you use a proof assistant. This may take more
time for you, but it makes my job easier.

Figure 3: You did not define A ⊨ ff. Should the words "and", "or",
etc. be interpreted in a classical or an intuitionistic meta-logic?

Definition 4.2, "there a finitely many substitutions": Do you mean
"there is a finite set of substitutions"?

Definition 4.2: How is ≤ defined?

Theorem 4.3: What do you mean by "fragment" and "decidable"? Can't you
prove full completeness (stated positively)?

Line 887: Please explain why these statements hold, with a focus on
the use of reachability in the entailment relation.

Line 901: Should D′ be defined with m, like C′, instead of ⟨m,r⟩?

Line 961, "The first responds only to the owner of private key a": Is
this right? It seems to me as if it responds to any message of the
form aenc(⟨m,pk(a)⟩,pk(c)). Do you mean that the response can only be
decrypted by the owner of private key a? How is this supposed to work?
The key a is bound in the server and not transmitted. Perhaps you
could include a couple of paragraphs that explain the basics of
modelling security/privacy using (variants of) the π-calculus.

Line 977: I assume that Q should be Broken_Server.

Line 1017, "Under all substitutions fresh for {u, v, w, a, b, c}": Is
this related to the requirement that the relation that you are
implicitly defining must be open?

Line 1022: The second occurrence of pk(a) should be pk(b).

Line 1023: The only occurrence of pk(a) should be pk(b).

Line 1043: Are readers supposed to know what blinding is?

Line 1050: The first occurrence of a should be a̅, right?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #37B
===========================================================================

Overall merit
-------------
A. Strong Accept

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
The applied $\pi$-calculus, introduced by Abadi and Fournet, extends the $\pi$-calculus with an equational theory of terms, augmenting the usual atomic names passed between processes. The intended application is to modelling cryptographic protocols, where the equational theory captures how processes can construct new messages and deduce information. The question of what the right notion of equivalence for the applied $\pi$-calculus is has not previously had a satsifactory answer, however. The original definition mistakenly allowed too many processes to be identified. Recent fixes have yielded equivalences that are not congruences, disallowing modular reasoning about privacy properties. This paper proposes a new equivalence, *quasi open-bisimilarity*, which is proved to be equivalent to the canonical definition (open barbed bisimilarity), but which is easier to reason about. A logical characterisation is also given, using an intuistionistic modal logic. The key technical contr
 ibution appears to be the notion of *open*ness through a definition of reachability between processes, which seems to capture a notion of what the context can learn given the currently public information.

Strengths
---------
- Seems to completely solve the problem of what the "right" equivalence for the applied $\pi$-calculus is, allowing modular reasoning about privacy properties.

- Modularity is particularly cool, and should help in the production of useful tools for the applied $\pi$-calculus.

- Technically sophisticated, but very well explained throughout. Full proofs given. I only found one place where there appeared to be some confusing typos (see below).

- Good examples that illustrate the technical definitions well.

- The concept of reachability may be useful in other work.

Weaknesses
----------
- Some of the example can be a bit hard to read due to the denseness of the $\pi$-calculus notation.

Comments for author
-------------------
I should preface this with the admission that I do not know very much about the applied $\pi$-calculus, and indeed did not know that the problem this paper solves was a problem until reading it. Nevertheless, as far as I can tell, this paper solves the problem completely, and moreover is very well written and easy to follow. Even the main proofs (pages 12 - 17) are relatively easy to follow (though I can't swear I didn't miss a small problem in the reasoning).

I did notice what I believe to be small typo / problem in the main definition: In Definition 3.2 (reachability), line 400, it is stated that $\sigma$ and $\rho$ are idempotent and fresh for $\mathrm{dom}(\theta)$. However, the non-example at the end of the next paragraph states that reachability does not apply here due to the freshness constraints, but I don't see how they apply? Should the $u$ be a $z$ in the active substitution here?

- Does reachability form a category? Is there a way to compose reachability substitutions?

- In the example on lines 442-450: I thought this example was meant to illustrate how openness or messages as channels are used? But they aren't mentioned?

- Line 683: "quasi-open bisimilarity" appears at the start of the line for no reason.

- Line 834 (Fig 3). There is a missing clause for ff.

- Line 838: In the clause for implication, is it necessary to apply the substitutions to the formulae? Is it not possible to incorporate the current substitution into the "world" and apply it when at an atomic formula?

- Line 943: Insert "The" before "sub-formula"

- Line 966: "observe" => "observer"

- Line 1047: "singnatures" => "signatures"

- Line 1050: First $a$ should have an overbar?

- Line 1162: "be" => "by"


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #37C
===========================================================================

Overall merit
-------------
B. Weak accept

Reviewer expertise
------------------
X. Expert

Paper summary
-------------

The paper develops a notion of open barbed bisimilarity for the
applied-pi calulus (a calculus used to model and analyse cryptographic
protocols). Then they develop a notion of quasi-open bisimilarity.
Such a notion is shown to coincide with the previous one and is actually
more amenable to automation since it avoids quantifying over all
contexts.

The main advantage of this new notion of equivalence (in comparison to
existing ones such as observational equivalence, trace equivalence) is
the fact that such a notion is a congruence, i.e. a relation closed by
all contexts. In comparison, observational equivalence only considers
closure by evaluation contexts (e.g. observational equivalence is not
closed by input prefixing).

This paper studies mostly the strong version of the equivalences, i.e.
the one in which tau
actions are taken into account. Similar notions can be obtained in
their weak version, and
these notions are shown to be stronger than the usual notion of
observational equivalence (and thus trace equivalence, the notion of
equivalence which is usually used to model privacy-type properties in
cryptographic protocols).
Thus, this new notion can be used as a proof technique to 
establish privacy-type security properties.

The authors also describe a modal logic (an extension of the
intuitionistic FM used to characterise open barbed bisimilarity in the
context of pi calculus) and they show that this modal
logic characterises the notion
of open barbed bisimilarity in the applied-pi calculus setting.

Strengths
---------
- A new notion of equivalence that could be useful to establish
  privacy-type properties in the context of security protocols
  analysis
- A notion providing a compositional approach to verifying
  cryptographic protocols.
- well-written paper

Weaknesses
----------

- the usefulness of this notion regarding security protocols
  verification remains to be justified.
- regarding composition, it is not clear whether this new notion is
  useful since protocols that we want to compose share some
  keys meaning that composition has to be done under name restrictions which
  is forbidden here.

Thus, from my point of view, the main critiscm is the fact that the
usefulness of their development is not demonstrated in a security
setting . However, I think that this is not a big issue to be published in a
venue like POPL.

Comments for author
-------------------


Main comments:
------------
A/ Mistake from [Abadi and Fournet 2001]
In the introduction, you mention a mistake in [Abadi and Fournet
2001]. I think that the process P can not be written in the syntax of
the original paper since, in [Abadi Fournet 2001], it is written "function symbols take
arguments and produce results of the base types only". Under such a
restriction, your counter-example is not valid anymore. Indeed, here you
assume the existence of a pair symbol whose first argument has channel
type.

Thus, from my point of view, this example should not be presented as a
mistake from [Abadi Fournet 2011].

B/ Static equivalence
I wonder whether there is a mistake in your definition of static
equivalence. Consider for instance, \nu x. {ok/y} and \nu y. {ok/x}.
According to your definition, the messages M and N can not rely on x
and y, therefore I think that static equivalence holds according to
your definition.


Then, at the bottom of page 8, you develop an example starting with
"For a less obvious example ...".  You say that the above extended
processes are statically equivalent whereas I think they are NOT.
To see that, consider the test 
aenc(adec(x1,x2),pk(x2))  == x1.
Such a test is satisfied by the process on the left but not by the
process on the right.


Lastly, on page 10, it is written:
{aenc(x,z)/v} and {aenc(y,z)/v} are statically equivalent. Again, I
think that they are NOT. The test v == aenc(x,z) can be used to
distinguish them.


C/ As several other papers, your aim is to propose a new notion of
equivalence that is amenable to automation and that can be used to
establish equivalence-based security properties. Diff-equivalence is
such a useful notion but unfortunately, this notion is often too
strong in practice. Here, I have to say that it is difficult to see
whether:
1/ your definition is more amenable to automation than the standard
notion (e.g. labelled bisimilarity or trace equivalence).
2/ your definition is less restricitve than diff-equivalence. In
other word, could your notion be used to establish equivalence where
the notion of diff-equivalence failed. 
Regarding 1/, you do not discuss this point. Regarding 2/, you provide
some examples but the one developed in Section 5.1 is now
automatically handled by an extension of the diff-equivalence [Cheval
Blanchet POST 2013]. I would therefore suggest you to devleop 
the e-passport example since it is an example on which
diff-equivalence fails.

More explanations regarding these points would be welcome.

D/ Characterisation.
I do not understand Theorem 4.3. What do you mean by "For fragments
of the applied-pi-calculus that are decidable" Which problem should be
decidable? You mention a proof in appendix but this proof is missing.


Minor comments
-------------

page 2: In your calculus, it seems that there is no distinction
between names and variables. However, it is a bit confusing since
sometimes you write nu x, y and sometimes, you prefer nu k,n.
Also, at several places, you  use the notion of name, e.g. page 4
"name binders", Fig 2 "define the names ..."
Could you clarify this? 

page 9: I found the notion of reachability difficult to understand.
Some illustrative examples would be welcome.

page 9, middle: "However, by extending the environment with a fresh
name, we have ..."
In the relation, I wonder why \nu x. has disappeared on the right. I
think that the active substitution {x/u} should be on the right, and
not on the left.

page 10:  "Critically, message y ranges over all permitted inputs"
I agree but I wondered whether this observation also holds form m. 

page 11: You say that, according to the original labelled bisimilarity
proposed in [Abadi Fournet 2001], the processes are labelled
bisimilar. This is wrong since this notion is only defined for closed
processes, and the process C' is not closed.

page 14 (line -3): Remove "quasi-open bisimilarty" before "Proof"

page 18, Definition 4.2: A equational --> An equational; there a
finitely --> there are finitely

page 19, line -3: I think that "x" should be replaced by "a" (two
occurrences).

page 20: an external observe --> an external observer

page 22, middle: R \models <a(u)> --> a should be replaced by
\overline{a}.

page 23, definition 6.2: Labelled bisimilarity is defined over CLOSED
extended processes.

page 24: obtained be --> obtained by

page 25: addessed --> addRessed

Questions for authors’ response
---------------------------------

I would like an answer to my point B, and in case the e-passport
example is detailed in a companion report, I would be more than happy
to read it. A clarification regarding Theorem 4.3 would be also welcome.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #37D
===========================================================================

Overall merit
-------------
C. Weak reject

Reviewer expertise
------------------
Z. No familiarity

Paper summary
-------------
The _applied_ $\pi$ calculus extends the $\pi$ calculus with explicit cryptographic primitives. Various flavors of bisimilarity are the standard way for verifying properties of $\pi$ calculus programs.

This paper argues that the _open barbed bisimilarity_---defined as the coarsest bisimilarity congruence---is the correct choice for verifying various properties in applied $\pi$ calculus. The authors show that _quasi-open bisimilarity_ is equivalent to open barbed bisimilarity, though the former is easier to reason with because of changes in how and where quantification happens.

Later, the paper characterizes open barbed bisimilarity using an intuitionistic model logic FM, modeling _f_ree input with equality _m_atching. The general correspondence between intuitionistic FM and quasi-open bisimilarity is due to Horne et al. 2018; this paper adapts their work to the applied $\pi$ calculus.

The authors explain that their work can be adapted from the strong bisimilarities described to weaker ones allowing internal $\tau$ steps.

Finally, several examples show that the reasoning principles in this work allow one to correctly identify privacy vulnerabilities and cryptographic attacks.

Strengths
---------
The technical work adapts Horne et al. 2018 to a new setting.

The notion of bisimilarity here can prove new properties.

Weaknesses
----------
There is very little in terms of concrete motivation.

No explicit contributions are claimed, making it difficult to evaluate the work.

There is little to no background.

The work is extremely technical, devoting a great deal of space to proofs.

Comments for author
-------------------
I'm by no means an expert on $\pi$ calculus, but I am familiar with it and am comfortable with simple notions of bisimilarity. I struggled to make heads or tails of this paper. Without claimed contributions, I'm left with the following understanding:

- Abadi et al. 2018 reframed the applied $\pi$ calculus, resolving some issues with messages and channels.
- Horne et al. 2018 showed open barbed bisimilarity and quasi-open bisimilarity coincide and related the latter to intuitionistic FM.
- This work takes Abadi et al.'s reframing and applies Horne et al.'s theory to it.

I would not be surprised at _all_ if I've misread things. But if that summary is indeed the case, it's not clear to me that this paper contributes results of interest in a way that is legible to a general POPL audience. My (limited) understanding of bisimilarity makes it clear that being able to reason with a bisimilarity that is a congruence is indeed a boon. But the fundamental result there seems due to Horne at al. L1209 says "This is the first logical characterisation of any bisimilarity congruence for any cryptographic calculus." Are there other contributions?

At a lower level, the examples were quite confusing. The cryptographic model is not at all clear. For example, at L134 "$m$ is an open term representing a known or guessable plaintext". If the attacker knows or can guess a plaintext, what is even going on? How is it the case that an attacker can discern a random nonce from a ciphertext, even if they already have the public key? My understanding is that it is very much the idea of encyrption that it is not, in general, easy to take a ciphertext $c$ and a public key $k$ and guess a plaintext $m$ such that $\mathsf{aenc}(m,k) = c$.

L39 "allowing messages as channels" should probably be "allowing channels as messages"

L966 "observer" -> "observer"?
L974 "later" -> "latter"
L1162 "be" -> "by"
L1184 "addessed"

Questions for authors’ response
---------------------------------
Please make concise and clear claims of contributions. If you are doing more than adapting Horne et al. 2018 to an applied $\pi$ calculus setting, please emphasize as much clearly!

Comments
===========================================================================

A1 Response by Ross Horne <ross.horne@gmail.com>
---------------------------------------------------------------------------
For Reviewer B:
---------------------

A/ I understand syntactic restrictions can avoid this, but many agree it's worrying that simple polyadic pi-calculus expressions could not previously be handled. The 2018 approach resolves this controversy. I can reword slightly, but it's healthy for the community if we come clean and lay this issue to rest.

B/ Regarding \nu x.{ok/y} and \nu y.{ok/x}, notice an invariant of a bisimulation is the domain of substitutions match; so your example would never occur when checking bisimilarity.

You are correct that converse equation [aenc(adec(m,n),pk(n))=m] is missing from Fig.1, required for the Bleichenbacher example, p.8. This fun example is perpendicular to results, so can be removed/corrected.

You are also correct that the example developed on page 10 should be \nu x.a<aenc(x,z)> and \nu x.a<aenc(<x,y>,z)>. The distinguishing test under substitution {z\pk(w)} becomes snd(adec(v,w))=y. Thank you.

C/ I'm sure you agree, constantly extending diff-equivalence in response to new problems is unsatisfactory. In contrast, here I prove quasi-open bisimilarity is fully saturated with all robust equations.

I try to avoid controversy, but it seems you are aware Arapinis'10 contains flaws. Correctly, there is an attack on Fig.6[Arapinis'10] described by the following FM-formula (in ASCII !/? represents output/input):

SystemFR|= <tau><c!u><d?get_challenge><c!nt><d?nt><c!y><d?y><c!z><tau><c!v><d?get_challenge><c!second_nt><d?second_nt><c!second_y><d?second_y><c!w>(w=6300)

Contrary to claims on p.14[Arapinis'10], SystemUK~SystemUK' does not hold; there is the following attack:

SystemUK|= <tau><tau><c!u><c!v><d?get_challenge><c!nt><d?nt><d?nt><c!y1><c!y2>(<d?y1><c!z1>(z2=/=error) /\ <d?y2><c!z2>(z2=/=error))

The above attack concurrently opens two sessions. The challenge nt intended for one reader is fed to the other; and responses y1,y2 are swapped. If there is no error, both are the same passport. The rebuttal window is too short to present resolutions. Note only, the discovery of the above is automatic using quasi-open bisimilarity. CSF'10+LICS'18 provides preliminary evidence of automation.

D/ Maybe you missed, popl19.hotcrp.com provides appendices in a separate PDF. The trick is, for decidable fragments, "not bisimilar" is defined even in an intuitionistic framework, c.f., CONCUR'17 and LICS'18. As you know, static equivalence is decidable for many useful message theories.


For Reviewer A/D:
-------------------------

Both worry about the contribution compared to LICS'18. I reassure you LICS'18 was written to support mismatch in the current submission, reinforcing mismatch with some machine checked proofs in the core system.

Even without mismatch, there has been no previous success lifting bisimilarity congruences to the applied pi-calculus. I try not to overstate results; however, providing a complete, robust and useful equivalence for one of the most powerful and widely used applied calculi should be a high-impact contribution. The modal logic itself is significant, since the problem of defining a modal logic characterising any bisimilarity for the applied pi-calculus had never really been solved (l.1165 is, as a token of respect, generous to Parrow'17). Having three semantics that coincide is an unprecedented case for correctness; and is useful since we know all attacks found can be described in the modal logic.

Regarding audience, I argue POPL is suitable, since I lay to rest problems debated for 18 years since POPL'01.

Note, I assume an intuitionistic meta-framework, so require no rule for the absurdity. Finally, contributions are explicit throughout.

Comment @A1 by Reviewer A
---------------------------------------------------------------------------
We decided not to accept this paper for publication in POPL 2019. Here are some points put forward in the discussion:
* Perhaps we misunderstood the contributions of the paper, but they seem somewhat incremental (applying the work of Horne et al. to the work of Abadi et al.).
* The paper could perhaps be improved (easier to understand, more accessible to a wider audience, and more obviously useful to the experts) by including more examples.




==> proofs.tex <==
\appendix

\section{Appendix}


The proof of Theorem~4.3, the completeness of open barbed bisimilarity with respect to modal logic $\FM$, is provided in this appendix.
The proof strategy follows closely techniques developed for the $\pi$-calculus~\cite{Ahn2017,Horne2018}.
The main novelty is the base case handling static equivalence and the compact approach enabled by extended processes, meaning all actions are treated in the same fashion.
%Extra care is required to ensure distinguishing formulae with inequalities that account properly for the set of names at each step in a distinguishing strategy (Def.~\ref{def:non-bisim}).

%We employ a form of \textit{disunifier} --- a substitution and set of names, witnessing a set of inequalities are satisfied.
%The subtlety is, unlike unifiers for equalities, there is not a single most general unifier representative of all solutions, but, instead finitely many most general disunifiers for any set of inequations.
%\begin{definition}
%Assume $\mathcal{D}$ is a set of pairs of distinct messages.
%Define $\vec{n} \vDash \mathcal{D}$ whenever, for all $M \not= N \in \mathcal{D}$, $\vec{n} \vDash M \not= N$.
%We say substitution $\sigma$ respects $\mathcal{D}$ whenever for all $M \not= N \in \mathcal{D}$, it is not the case that $M\sigma =_E N\sigma$.
%A pair ($\sigma, \vec{m}$) consisting of a substitution and set of names is a disunifier for $\vec{n}$ and $\mathcal{D}$
%whenever $\sigma$ respects $\vec{n}$ and $\mathcal{D}$ and $\vec{m},\vec{n} \vDash \mathcal{D}\sigma$.
%A disunification set $(\sigma_i, \vec{n}_i)$ for $\vec{m}$ and $\mathcal{D}$ is such that $(\sigma_i, \vec{n}_i)$ is a disunifier for $\vec{m}$ and $\mathcal{D}$. The disunification set is complete if for all disunifiers $(\theta, \vec{k})$ for $\vec{m}$ and $\mathcal{D}$, there exists $i$ such that $\sigma_i \leq \theta$ and $\vec{n}_i \subseteq \vec{k}$ (upto renaming of $\vec{n}_i$). A complete disunification set is minimal, whenever there is no $i$ and $j$ such that $\sigma_i \leq \sigma_j$ and $\vec{n}_i \subseteq \vec{n}_j$.
%\end{definition}




\textbf{Theorem~4.3 can now be established.}
\begin{proof}
\input{modal_proof}
\end{proof}


